Governing Governance: A Formal Framework for Analysing Institutional Design and Enactment Governance

This dissertation is motivated by the need, in today's globalist world, for a precise way to enable governments, organisations and other regulatory bodies to evaluate the constraints they place on themselves and others. An organisation's modus operandi is enacting and fulfilling contracts between itself and its participants. Yet, organisational contracts should respect external laws, such as those setting out data privacy rights and liberties. Contracts can only be enacted by following contract law processes, which often require bilateral agreement and consideration. Governments need to legislate whilst understanding today's context of national and international governance hierarchy where law makers shun isolationism and seek to influence one another. Governments should avoid punishment by respecting constraints from international treaties and human rights charters. Governments can only enact legislation by following their own, pre-existing, law making procedures. In other words, institutions, such as laws and contracts are designed and enacted under constraints.

==> appendices/appendices.tex <==
\chapter*{Appendices}

{\color{tck-grey}These appendices accompany the dissertation titled Governing Governance: A Formal Framework for Analysing Institutional Design and Enactment Governance by Thomas C. King - Technical University of Delft}

\newpage

\section{Multi-Level Governance Computational Framework Proofs}
\label{secAppCompProofs}

\subsection{Deontological Counts-as Soundness Proof}
\label{proofAbstraction}
\begin{proof}{Lemma~\ref{theoremAbstraction}} We need to show that $S^{i}_{j} \subseteq \overline{\textit{DC}}^{i}(S^{i}_{j})$ and $\overline{\textit{DC}}^{i}(S^{i}_{j}) \subseteq S^{i}_{j}$. Each case is dealt with separately:
\begin{enumerate}
\item $S^{i}_{j} \subseteq \overline{\textit{DC}}^{i}(S^{i}_{j})$ - If $f \in S^{i}_{j}$ then $f \in \overline{\textit{DC}}^{i}(S^{i}_{j})$ due to monotonicity of $\overline{\textit{DC}}^{i}$.
\item $\overline{\textit{DC}}^{i}(S^{i}_{j}) \subseteq S^{i}_{j}$ - given that if $\langle N, n \rangle \in \textit{DC}(S^{i}_{j})$ and $S^{i}_{j} \models N$ then $n \in \overline{\textit{DC}}^{i}(S^{i}_{j})$, we need to show that $n \in S^{i}_{j}$. By construction of $S^{i}_{j}$ we know that $n \in S^{i}_{j}$ iff $M_{P} \models \asp{holdsat(} n, \textit{In}^{i}, j)$, in turn we know $M_{P} \models \asp{holdsat(} n, \textit{In}^{i}, j)$ iff $\asp{holdsat(} n, \textit{In}^{i}, j)$ is an atom in the head of an applied rule. We show for every $\langle N, n \rangle \in \textit{DC}(S^{i}_{j})$ and $n$ given in Definition~\ref{defDC}, under the assumption that $S^{i}_{j} \models N$ that there is an applied rule $r$ with the atom $\asp{holdsat(} n, \textit{In}^{i}, j) = H(r)$ in the head. By induction on two counters:
\begin{enumerate}[label*=\arabic*.]
\item \label{proofDCBCaseObl} \textbf{Base case 1:} According to \ref{eqDC1} $N = \{ \textit{obl}(a, d) \}$ and $n = \textit{obl}(b, d)$ where $b \in \pazocal{E}^{i} \cup \pazocal{F}^{i}$. From \ref{eqDC1} we know that $\exists a \in \pazocal{E}^{i} \pazocal{F}^{i}$ and $\exists X \in \pazocal{X}^{i}$ s.t. $S^{i}_{j} \models X$ and $b \in \pazocal{G}^{i}(X, a) \cup \pazocal{D}^{i}(X, a)$, and $n \in \pazocal{F}^{i}_{\textit{anorm}}$. Thus, the conditions on the left hand side of transformation \ref{eqASPDCATrans1} or are met and therefore we have an AnsProlog rule $\asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i, I \asp{) :- }$ \\$\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{),} \asp{nifluent(}\textit{obl(}b, d\asp{)}, \textit{In}^{i} \asp{),} \asp{instant(I).}$ or the conditions of transformation \ref{eqASPDCATrans5} are met and we have an AnsProlog rule \\$\asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i, I \asp{) :- }
\textit{CN}\asp{,} \textit{C} \asp{,} \asp{nifluent(}\textit{obl(}b, d\asp{)}, \textit{In}^{i} \asp{),} \asp{instant(I).}$. Since according to \ref{eqASPSemTrans16} \\$\asp{instant(}j\asp{).} \in \Pi^{\textit{base(k)}}$ is a fact, therefore $M_{P} \models \asp{instant(}j\asp{)}$ and we have a ground rule $r = \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i, j \asp{) :- }$ \\$
\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, j\asp{),} \asp{nifluent(}\textit{obl(}b, d\asp{)}, \textit{In}^{i} \asp{),} \asp{instant(}j\asp{).} \in P^{*}$ or a ground rule $r = \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i, j \asp{) :- }$ \\$
\textit{CN}\asp{,} \textit{C} \asp{,} \asp{nifluent(}\textit{obl(}b, d\asp{)}, \textit{In}^{i} \asp{),} \asp{instant(}j\asp{).} \in P^{*}$ where \\ $\textit{CN} = \{\textit{EX(obl(a, d),} \pazocal{I}^{i}) \asp{:} \textit{EX(X}^{i}, \pazocal{I}^{i})\asp{;}\}$ and $C = \asp{1\{} \textit{CN} \asp{\}}$. We need to show \\$\forall l \in B(r) : M_P \models l$:
\begin{enumerate}[label*=\arabic*.]
\item $\textit{CN}$ - According to \ref{eqASPDCATrans1} $\textit{CN} = \{\textit{EX(obl(a, d),} \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;}\}$ is a singleton containing a conditional literal and according to Definition~\ref{defASPDCATrans} \\$\textit{EX(obl(a, d),} \pazocal{I}^{i}) \asp{:} \textit{EX(X}^{i}, \pazocal{I}^{i})\asp{;} \in B(r)$. We will show that if $M_P \models \textit{EX(X}^{i}, \pazocal{I}^{i})\asp{;}$ then assuming $S^{i}_{j} \models N$ that $M_P \models \textit{EX(obl(a, d),} \pazocal{I}^{i})$:
\begin{enumerate}[label*=\arabic*.]
\item By \ref{eqASPDCATrans1} or \ref{eqASPDCATrans5} $\textit{CN}$ is constructed such that if \\$\textit{EX(obl(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;} \in \textit{CN}$ then $a \in \pazocal{E}^{i} \cap \pazocal{F}^{i}, X \in \pazocal{X}^{i}$ s.t. $b \in \pazocal{G}^{i}(X, a) \cap \pazocal{D}^{i}(X, $.
\item If $X = \emptyset$ then $\textit{EX(X, } \pazocal{I}^{i})$ translates to $\asp{\#true}$ and it is always the case that $M_P \models \asp{\#true}$ and since $X = \emptyset$ we have $S^{i}_{j} \models X$.
\item If $X \neq \emptyset$ and $M_P \models \textit{EX(X, } \pazocal{I}^{i})$ then since $\textit{EX(X, } \pazocal{I}^{i})$ translates to \\$\asp{holdsat}/3$ literals, by construction of $S^{i}_{j}$ it is the case that $S^{i}_{j} \models X$. 
\item By $N$ we have $N = \{ \textit{obl}(a,d)\}$ and assuming $S^{i}_{j} \models N$ we have $S^{i}_{j} \models \textit{obl}(a,d)$ and by construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(obl(a,d), } \pazocal{I}^{i})$.
\item By 2.1.1.1., 2.1.2. and 2.1.1.3. and construction and construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(X}^{i}, \pazocal{I}^{i})\asp{;}$ and with 2.1.1.4 we have $M_P \models \textit{EX(obl(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})$.
\end{enumerate}
We have shown that for all $\textit{EX(obl(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;}$ in $\textit{CN} : M_P \models \textit{EX(X, } \pazocal{I}^{i})$ it is the case that  $\textit{obl}(a,d) \in N$ and therefore that $M_P \models \textit{EX(obl(a,d), } \pazocal{I}^{i})$, and $M_P \models \textit{CN}$.
\item $C$ - According to \ref{eqASPDCATrans1} $C = \asp{1\{} \textit{CN} \asp{\}}$, by translation \\$C = \asp{1\{} \asp{holdsat(obl(a, d),} \pazocal{I}^{i}, \asp{I)} : \textit{EX(X}^{i}, \pazocal{I}^{i}) \asp{;\}}$. $C$ is true if at least one element is true, under the semantics of aggregates we need to show $M_P \models \textit{EX(obl(a, d)}, \pazocal{I}^{i})$ and $M_P \models \textit{EX(X}, \pazocal{I}^{i})$.
\begin{enumerate}[label*=\arabic*.]
\item We have already established that $N$ is constructed s.t. $X \in \pazocal{X}^{i}$ and $S^{i}_{j} \models X$. By construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(X}^{i}, \pazocal{I}^{i})$. 
\item Since $\asp{holdsat(obl(a, d),} \pazocal{I}^{i}, \asp{I)} : \textit{EX(X}^{i}, \pazocal{I}^{i}) \asp{;} \in \textit{CN}$ by 2.1.2.1 and 2.1.1.5 we have \\$M_P \models \asp{holdsat(obl(a, d),} \pazocal{I}^{i}, \asp{I)}$.
\end{enumerate}
By 2.1.2.1 and 2.1.2.2 we have $M_P \models C$.
\item In the case that $r$ is produced by \ref{eqASPDCATrans1}  $\asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, j\asp{)}$ - since $N=\{ \textit{obl(a,d)} \}$ the condition of its construction $S^{i}_{j} \models \textit{pow}(b)$ according to \ref{eqDC1} holds. By construction of $S^{i}_{j}$ we know $M_{P} \models \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, j\asp{)}$.
\item $\asp{nifluent(}\textit{obl(}b, d\asp{)}, \textit{In}^{i})$ - true by $\textit{obl(}b, d\asp{)} \in \pazocal{F}_{\textit{anorm}}$ and \ref{eqASPMLTrans4}.
\item $\asp{instant(}j\asp{)}$ - According to \ref{eqASPSemTrans16} $\asp{instant(}j\asp{).} \in \Pi^{\textit{base(k)}}$ is a fact and therefore $M_{P} \models \asp{instant(}j\asp{)}$.
\end{enumerate}
We have shown that for any $\langle N, n \rangle \in \textit{DC}(S^{i}_{j})$ where $N = \{ \textit{obl}(a, d) \}$ and $n = \textit{obl}(b, d)$ where $b \in \pazocal{E}$ that we have a ground rule \\$r = \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i, j \asp{) :- }
\textit{CN}\asp{,} \textit{C} \asp{,}\\ \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, j\asp{),} \asp{instant(}j\asp{).} \in P^{*}$ or a ground rule \\ $r = \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i, j \asp{) :- } \textit{CN}\asp{,} \textit{C} \asp{,}\\ \asp{instant(}j\asp{).} \in P^{*}$ and that assuming $S^{i}_{j} \models N$ then $\forall l \in B(r) : M_P \models l$ and thus $M_P \models H(r)$ and by construction $S^{i}_{j} \models n$.
\item \label{proofDCBCasePro} \textbf{Base case 2:} According to \ref{eqDC2} $N = \{ \textit{pro}(a_{0}, d), ..., \textit{pro}(a_{l}, d) \}$ and $n = \textit{pro}(b, d)$ where $b \in \pazocal{E}$. We know that from Definition~\ref{defDC} $N \neq \emptyset$ and from \ref{eqDC1} $N$ is constructed as $N = \{ \textit{pro}(a, d) \mid \; \exists X, a : X \in \pazocal{X}^{i} \wedge a \in \pazocal{E}_{\textit{inst}}^{i} \wedge n^{\prime} = \textit{pro}(b, d) \wedge S^{i}_{j} \models X \wedge  b \in \pazocal{G}^{i}(X, a) \wedge S^{i}_{j} \models \textit{pow}(b) \}$ thus on the left hand side of the transformations \ref{eqASPDCATrans2} and \ref{eqASPDCATrans6} the set $\textit{CN}$ is non-empty and since $n \in \pazocal{F}^{i}_{\textit{anorm}}$ all conditions of \ref{eqASPDCATrans2} or \ref{eqASPDCATrans6} are met. Therefore we have an AnsProlog rule $\asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i, I \asp{) :- }$ \\
$\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{),} \asp{nifluent(}\textit{pro(}b, d\asp{),} \asp{instant(}I\asp{).}$ or an AnsProlog rule $\asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i, I \asp{) :- }$ \\ $\textit{CN}\asp{,} \textit{C} \asp{,} \asp{nifluent(}\textit{pro(}b, d\asp{),} \asp{instant(}I\asp{).}$ and since according to \ref{eqASPSemTrans16} $\asp{instant(}j\asp{).} \in \Pi^{\textit{base(k)}}$ is a fact, we have $M_{P} \models \asp{instant(}j\asp{)}$ and a ground rule \\$r = \asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i, j \asp{) :- }$ \\
$\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, j\asp{),} \asp{nifluent(}\textit{pro(}b, d\asp{),} \asp{instant(}j\asp{).} \in P^{*}$ or a ground rule \\ $r = \asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i, j \asp{) :- }
\textit{CN}\asp{,} \textit{C} \asp{,} \asp{nifluent(}\textit{pro(}b, d\asp{),} \asp{instant(}j\asp{).} \in P^{*}$. We need to show each term in the body of $r$ is true in $M_{P}$ s.t. $\forall l \in B(r) : M_{P} \models l$:
\begin{enumerate}[label*=\arabic*.]
\item \textit{CN} - According to \ref{eqASPDCATrans2} or \ref{eqASPDCATrans6} $\textit{CN} = \{ \textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;} \mid a \in \pazocal{E}^{i} \cap \pazocal{F}^{i}, X \in \pazocal{X}^{i}, b \in \pazocal{G}^{i}(X, a) \cap \pazocal{D}^{i}(X, a) \}$ is a set of conditional literals comma-delimited in the rule $r$ according to definition~\ref{defASPDCATrans} s.t. \\$\forall \textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;} \in \textit{CN} : \textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;} \in B(r)$. \\ We will show every conditional literal in $\textit{CN}$ is true s.t. \\$\forall  \textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;} \in \textit{CN}$ if $M_P \models \textit{EX(X, } \pazocal{I}^{i})$ then assuming $S^{i}_{j} \models N$ that $M_P \models \textit{EX(pro(a,d), } \pazocal{I}^{i})$.
\begin{enumerate}[label*=\arabic*.]
\item By \ref{eqASPDCATrans2} or \ref{eqASPDCATrans6} $\textit{CN}$ is constructed such that if $\textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;}$ \\ $\in \textit{CN}$ then $a \in \pazocal{E}^{i} \cap \pazocal{F}^{i}, X \in \pazocal{X}^{i}$ s.t. $b \in \pazocal{G}^{i}(X, a) \cap \pazocal{D}^{i}(X, a)$. 
\item If $X = \emptyset$ then $\textit{EX(X, } \pazocal{I}^{i})$ translates to $\asp{\#true}$ for which it is always the case $M_P \models \asp{\#true}$ and since $X = \emptyset$ we have $S^{i}_{j} \models X$. 
\item If $X \neq \emptyset$ and $M_P \models \textit{EX(X, } \pazocal{I}^{i})$ then since $\textit{EX(X, } \pazocal{I}^{i})$ translates to \\$\asp{holdsat}/3$ literals, by construction of $S^{i}_{j}$ it is the case that $S^{i}_{j} \models X$. 
\item If $M_P \models \textit{EX(X, } \pazocal{I}^{i})$ with 2.1.1. we have $b \in \pazocal{G}^{i}(X, a)$ and by By 2.1.2 and 2.1.3. we have $S^{i}_{j} \models X$ therefore by construction of $N$ we have $\textit{pro}(a,d) \in N$. 
\item Under the assumption that $S^{i}_{j} \models N$, $\textit{pro}(a,d) \in S^{i}_{j}$ and therefore by construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(pro(a,d), } \pazocal{I}^{i})$. 
\item By 2.1.2., 2.1.3 and 2.1.4. by construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(pro(a,d), } \pazocal{I}^{i})$ \\ $\asp{:} \textit{EX(X, } \pazocal{I}^{i})$.
\end{enumerate}
We have shown that for all $\textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;}$ in $\textit{CN}$ if$M_P \models \textit{EX(X, } \pazocal{I}^{i})$  then \\$M_P \models \textit{EX(pro(a,d), } \pazocal{I}^{i})$, and $M_P \models \textit{CN}$.
\item $C$ - According to \ref{eqASPDCATrans2} or \ref{eqASPDCATrans6} $C = \asp{1\{} \textit{CN} \asp{\}}$, is an aggregate which is true if at least one element is true, under the semantics of aggregates we need to show $\exists \textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;} \in \textit{CN} : M_P \models \textit{EX(pro(a, d)}, \pazocal{I}^{i}) \wedge M_P \models \textit{EX(X, } \pazocal{I}^{i})$. 
\begin{enumerate}[label*=\arabic*.]
\item By Definition~\ref{defDC} $N \neq \emptyset$ and by \ref{eqDC2} $N$ is constructed as  $\{ \textit{pro}(a, d) \mid \; \langle A, b \rangle \in \pazocal{A}^{i}(S^{i}) \wedge a \in A \}$ and if by \ref{eqCA1} $\langle A, b \rangle \in \pazocal{A}^{i}(S^{i})$ then $S \models \textit{pow}(b) $. Therefore we know that by \ref{eqCA1} or \ref{eqCA2} $\exists X, a : X \in \pazocal{X}^{i} \wedge a \in \pazocal{E}^{i} \cap \pazocal{F}^{i} \wedge S \models X \wedge  b \in \pazocal{G}^{i}(X, a) \cap \pazocal{D}^{i}(X, a)$.
\item By 2.2.2.1. we have $\textit{pro}(a,d) \in N$ and by construction of $\textit{CN}$ in \ref{eqASPDCATrans2} we have that there exists $\textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;} \in \textit{CN}$ such that $S^{i}_{j} \models X$.
\item By construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(X, } \pazocal{I}^{i})$. 
\item Assuming $S^{i}_{j} \models N$, by 2.2.2.1. and by construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(pro(a,d), } \pazocal{I}^{i})$
\end{enumerate}
We have shown by 2.2.2.3 and 2.2.2.4 that there exists $\textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:}$ \\ $\textit{EX(X, } \pazocal{I}^{i})\asp{;}$ in $\textit{CN}$ such that $M_P \models \textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} \textit{EX(X, } \pazocal{I}^{i})\asp{;}$ and therefore that $M_P \models C$.
\item For the case that $\langle A, b \rangle \in \pazocal{A}^{i}(S^{i})$ by \ref{eqCA1} $\asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, j\asp{)}$ - since by the condition of constructing $N$ we have $S^{i}_{j} \models \textit{pow}(b)$ according to \ref{eqDC2}. By construction of $S^{i}_{j}$ we know $M_{P} \models \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, j\asp{)}$.
\item $\asp{nifluent(}\textit{pro(}b, d\asp{)}, \textit{In}^{i})$ - true by $\textit{pro(}b, d\asp{)} \in \pazocal{F}_{\textit{anorm}}$ and \ref{eqASPMLTrans4}.
\item $\asp{instant(}j\asp{)}$ - According to \ref{eqASPSemTrans16} $\asp{instant(}j\asp{).} \in \Pi^{\textit{base(k)}}$, a fact and therefore $M_{P} \models \asp{instant(}j\asp{)}$.
\end{enumerate}
We have shown that for any $\langle N, n \rangle \in \textit{DC}(S^{i}_{j})$ where $n = \textit{pro}(b, d)$ and $b \in \pazocal{E}$ then we have a ground rule $r = \asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i, j \asp{) :- }$ \\
$\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, j\asp{),} \asp{instant(}j\asp{).} \in P^{*}$ and that assuming $S^{i}_{j} \models N$ then $\forall l \in B(r) : M_P \models l$ and thus $M_P \models H(r)$ and by construction $S^{i}_{j} \models n$.
\item \label{proofDCInductiveHyp} \textbf{Inductive hypothesis:} Let $\langle N, n^{\prime} \rangle \in \textit{DC}(S^{i}_{j})$ then $\exists r \in \Pi^{\textit{abstr}}$ s.t. $r = \asp{holdsat(}n^{\prime}, \textit{In}^i, I \asp{) :- }\\
\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{),} \asp{nifluent(}n^{\prime}, \textit{In}^{i}), \asp{instant(}I\asp{).}$ or $r = \asp{holdsat(}n^{\prime}, \textit{In}^i, I \asp{) :- }\\
\textit{CN}\asp{,} \asp{nifluent(}n^{\prime}, \textit{In}^{i}), \textit{C}\asp{.}$ where $\textit{CN}$ is a set of conditional literals s.t. \\$\forall l \in C : l = \textit{EX(n}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;}, n \in N, X \in \pazocal{X}^{i}$ and $\textit{CN} \neq \emptyset$, and $C$ is an aggregate s.t. $C = \asp{1\{} \textit{CN} \asp{\}}$. The following properties hold:
\begin{enumerate}[label*=\arabic*.]
\item If $\textit{EX(n}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}$ and $M_P \models \textit{EX(X}, \pazocal{I}^{i})$ then assuming $S^{i}_{j} \models N$ by construction of $S^{i}_{j}$ it is the case that $M_P \models \textit{EX(n}, \pazocal{I}^{i})$. Therefore $M_P \models \textit{CN}$.
\item Assuming $S^{i}_{j} \models N$ then $\exists \textit{EX(n}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}$ such that $M_P \models  \textit{EX(X}, \pazocal{I}^{i})$ and $M_P \models \textit{EX(n}, \pazocal{I}^{i})$ therefore $M_P \models C = \asp{1\{} \textit{CN} \asp{\}}$.
\item In the case that $\asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, \asp{I)} \in B(r)$ it is the case that $M_P \models \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, \asp{I)}$.
\item $M_P \models \asp{nifluent(}n^{\prime}, \textit{In}^{i})$
\item It is the case that $M_P \models \asp{instant(}\asp{I)}$.
\end{enumerate}
Thus, assuming $S^{i}_{j} \models N$ then $M_P \models \asp{holdsat(}n^{\prime}, \textit{In}^i, I \asp{)}$ and by construction of $S^{i}_{j}$ it is the case that $n^{\prime} \in S^{i}_{j}$.
\item \textbf{Inductive step 1:} Let $\langle N^{\prime}, n^{\prime} \rangle \in \textit{DC}(S^{i}_{j})$ where $n^{\prime} = \textit{obl}(b, d)$ and $b \in \pazocal{F}^{i}_{\textit{anorm}}$. According to the conditions of \ref{eqDC1} $\exists \langle N, b \rangle \in \textit{DC}(S^{i}_{j})$. By the inductive hypothesis \\$\exists r \in P^{*}$ s.t. $r = \asp{holdsat(}b, \textit{In}^i, I \asp{) :- }$ \\ $\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{),} \asp{nifluent(}b, \textit{In}^{i}), \asp{instant(}I\asp{).}$ or \\$r = \asp{holdsat(}b, \textit{In}^i, I \asp{) :- }$ \\
$\textit{CN}\asp{,} \textit{C} \asp{,} \asp{nifluent(}b, \textit{In}^{i}), \asp{instant(}I\asp{).}$. Therefore the conditions of \ref{eqASPDCATrans3} are met and we have a rule $r^{\prime} \in \Pi^{\textit{abstr}}$ such that $r^{\prime} = \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i \asp{,I) :- }\\\textit{CN}^{\prime}, C^{\prime} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}\asp{, I),} \asp{nifluent(obl(}b, d\asp{)}, \textit{In}^{i}), \asp{instant(I).}$ or $r^{\prime} = \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i \asp{,I) :- }\\\textit{CN}^{\prime}, C^{\prime} \asp{,} \asp{nifluent(obl(}b, d\asp{)}, \textit{In}^{i}), \asp{instant(I).}$. We will now show that assuming $S^{i}_{j} \models N^{\prime}$ each body literal in $r^{\prime}$ is true.
\begin{enumerate}[label*=\arabic*.]
\item $\textit{CN}^{\prime}$ - According to \ref{eqASPDCATrans3} $\textit{CN}^{\prime} = \{ \textit{EX(obl(a,d), } \pazocal{I}^{i}) \asp{:} c\asp{;} \mid \asp{holdsat(}a, \textit{In}^i \asp{,I) : } c\asp{;} \in \textit{B}(r) \},$ we will show that if $S^{i}_{j} \models c$ then assuming $S^{i}_{j} \models N$ that $S^{i}_{j} \models \textit{EX(obl(a,d), } \pazocal{I}^{i})$.
\begin{enumerate}[label*=\arabic*.]
\item By the inductive hypothesis 2.3. the only conditional literals in $r$ are in $\textit{CN}$ s.t. \\$\asp{holdsat(}a, \textit{In}^i \asp{,I) : } c \asp{;} \in \textit{B}(r)$ iff $\asp{holdsat(}a, \textit{In}^i \asp{,I) : } c \asp{;} \in \textit{CN}$, therefore \\$\textit{CN}^{\prime} = \{ \textit{EX(obl(a,d), } \pazocal{I}^{i}) \asp{:} c \asp{;} \mid \asp{holdsat(}a, \textit{In}^i \asp{,I) : } c\asp{;} \in \textit{CN} \}$. 
\item By the inductive hypothesis 2.3.1. if $\textit{EX(a}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}$ and $M_P \models \textit{EX(X}, \pazocal{I}^{i})$ then assuming $S^{i}_{j} \models N$ by construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(a}, \pazocal{I}^{i})$. Therefore $\forall \textit{EX(a}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}$ such that $M_P \models \textit{EX(X}, \pazocal{I}^{i})$ we have $a \in N$. 
\item According to \ref{eqDC2} $N^{\prime}$ is constructed as $N^{\prime} = \{ \textit{obl}(a, d) \mid \; \exists a : a \in N \}$ by 2.4.1.2. and by construction of $\textit{CN}^{\prime}$ in \ref{eqASPDCATrans3} we have for all $\textit{EX(obl(a, d)}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;}$ in $\textit{CN}$ if $M_P \models \textit{EX(X}, \pazocal{I}^{i})$ then $\textit{obl(a, d)} \in N^{\prime}$. 
\item Assuming $N^{\prime} S^{i}_{j} \models N^{\prime}$ then we have $M_P \models \textit{EX(obl(a, d)}, \pazocal{I}^{i}$ and by 2.4.1.3. we have $M_P \models \textit{CN}^{\prime}$.
\end{enumerate}
\item  According to \ref{eqASPDCATrans3} $C^{\prime} = \asp{1\{}\textit{CN}^{\prime}\asp{\}}$, we will show that at least one element of $C^{\prime}$ is modelled by $M_P$ and therefore $C^{\prime}$ is true.
\begin{enumerate}[label*=\arabic*.]
\item By the inductive hypothesis 2.3.1. we have $\exists \textit{EX(a}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}$ such that $M_P \models  \textit{EX(X}, \pazocal{I}^{i})$. 
\item By 2.4.1. $M_P \models \textit{CN}^{\prime}$ with 2.4.2.1. there exists $\textit{EX(obl(a, d)}, \pazocal{I}^{i})$ \\ $\asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}$ such that $M_P \models\textit{EX(obl(a, d)}, \pazocal{I}^{i})$. 
\item Under the semantics of aggregates one element of $C$ must be true for $C$ to be true, together with 2.4.2.2. we have $M_P \models C = \asp{1\{} \textit{CN} \asp{\}}$.
\end{enumerate}
\item By the inductive hypothesis if $\asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{)} \in B(r)$ then $M_P \models \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{)}$.
\item By the inductive hypothesis $M_P \models \asp{nifluent(}\textit{obl(}b, d\asp{)}, \textit{In}^{i})$.
\item By the inductive hypothesis it is the case that $M_P \models \asp{instant(}I\asp{)}$.
\end{enumerate}
Thus, we have shown assuming $S^{i}_{j} \models N^{\prime}$ then $\forall l \in B(r^{\prime}) : M_P \models l$, therefore $M_P \models \asp{holdsat(}n^{\prime}, \textit{In}^i, I \asp{)}$ and by construction of $S^{i}_{j}$ it is the case that $n^{\prime} \in S^{i}_{j}$.
\item \textbf{Inductive step 2:} Let $\langle N^{\prime}, n^{\prime} \rangle \in \textit{DC}(S^{i}_{j})$ where $n^{\prime} = \textit{pro}(b, d)$ and $b \in \pazocal{F}^{i}_{\textit{anorm}}$. According to the conditions of \ref{eqDC2} $N^{\prime}$ is constructed as $\{ \textit{pro}(a, d) \mid \; \exists \langle N, b \rangle, a : \langle N, b \rangle \in \textit{DC}(S^{i}_{j}) \wedge a \in N \}$, $N^{\prime} \neq \emptyset$ and by the inductive hypothesis \\$\forall \langle N, b \rangle \in \textit{DC}(S^{i}_{j}) : \exists r \in P^{*}$ s.t. $r = \asp{holdsat(}b, \textit{In}^i, I \asp{) :- }$ \\ $
\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{),} \asp{nifluent(}\textit{b} \asp{,} \textit{In}^{i}), \asp{instant(}I\asp{).}$ or \\$r = \asp{holdsat(}b, \textit{In}^i, I \asp{) :- }
\textit{CN}\asp{,} \textit{C} \asp{,} \asp{nifluent(}\textit{b} \textit{In}^{i}), \asp{instant(}I\asp{).}$. Therefore the conditions of \ref{eqASPDCATrans4} are met and we have a rule \\$r^{\prime} \in \Pi^{\textit{abstr}}$ such that $r^{\prime} = \asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i \asp{,I) :- }\\\textit{CN}^{\prime}, C^{\prime} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}\asp{, I),} \asp{nifluent(}\textit{pro(}b, d\asp{)}, \textit{In}^{i}), \asp{instant(I).}$ or a rule \\$r^{\prime} \in \Pi^{\textit{abstr}}$ such that $r^{\prime} = \asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i \asp{,I) :- }\\\textit{CN}^{\prime}, C^{\prime} \asp{,} \asp{nifluent(}\textit{pro(}b, d\asp{)}, \textit{In}^{i}), \asp{instant(I).}$. We will now show that assuming $S^{i}_{j} \models N^{\prime}$ each body literal in $r^{\prime}$ is true.
\begin{enumerate}[label*=\arabic*.]
\item $\textit{CN}^{\prime}$ - According to \ref{eqASPDCATrans4} $\textit{CN}^{\prime} = \{ \textit{EX(pro(a,d), } \pazocal{I}^{i}) \asp{:} c\asp{;} \mid r \in R,
\asp{holdsat(}a, \textit{In}^i \asp{,I) : }$ \\ $c\asp{;} \in B(r) \}$ where $R = \{ r \in \Pi^{\textit{abstr}} : \textit{H}(r) = \asp{holdsat(}b\asp{,} \textit{In}^{i}, \asp{I)} \}$. We will show that if $S^{i}_{j} \models c$ then assuming $S^{i}_{j} \models N^{\prime}$ that $S^{i}_{j} \models \textit{EX(pro(a,d), } \pazocal{I}^{i})$.
\begin{enumerate}[label*=\arabic*.]
\item By the inductive hypothesis, and since according to Definition~\ref{defASPDCATrans} there are no other rules in $\Pi_{\textit{abstr}}$ not covered by the base cases 1 and 2 and the inductive hypothesis we have the following bi-directional property $\langle N, b \rangle \in \textit{DC}(S^{i}_{j})$ iff $\exists r \in P^{\textit{abstr}}$ s.t. \\$r = \asp{holdsat(}b, \textit{In}^i, I \asp{) :- }
\textit{CN}\asp{,} \textit{C} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{),} \asp{instant(}I\asp{).}$.
\item By the inductive hypothesis 2.3.1. for all \\$r \in P^{\textit{abstr}}$ s.t. $H(r) = \asp{holdsat(}b, \textit{In}^i, I \asp{)}$ if $\textit{EX(a}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}$ and $M_P \models \textit{EX(X}, \pazocal{I}^{i})$ then $a \in N$
\item According to \ref{eqDC2} $N^{\prime}$ is constructed as $N^{\prime} = \{ \textit{pro}(a, d) \mid \exists \langle N, b \rangle, a : \langle N, b \rangle \in \textit{DC}(S^{i}_{j}) \wedge a \in N \}$ and by 2.5.1.2. we have for all \\$\textit{EX(pro(a, d)}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;}$ in $\textit{CN}^{\prime}$ if $S^{i}_{j} \models X$ then by construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(X}, \pazocal{I}^{i})$, assuming $N^{\prime} \subseteq S^{i}_{j}$ we have $M_P \models \textit{EX(pro}(b, d), \pazocal{I}^{i})$. Therefore, $M_P \models \textit{CN}^{\prime}$.
\end{enumerate}
\item According to \ref{eqASPDCATrans4} $C^{\prime} = \asp{1\{}\textit{CN}^{\prime}\asp{\}}$ we will show that at least one element of $C^{\prime}$ is modelled by $M_P$ and therefore $C^{\prime}$ is true.
\begin{enumerate}[label*=\arabic*.]
\item By the inductive hypothesis 2.3.2. we have $\exists \textit{EX(a}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime}$ such that $M_P \models  \textit{EX(X}, \pazocal{I}^{i})$. 
\item By 2.5.1. $M_P \models \textit{CN}^{\prime}$ and $\textit{EX(pro(a, d)}, \pazocal{I}^{i}) \asp{:} \textit{EX(X}, \pazocal{I}^{i})\asp{;} \in \textit{CN}$ and by 2.5.2.1 we have $M_P \models\textit{EX(X}, \pazocal{I}^{i})$ therefore under the semantics of aggregates we have $M_P \models C = \asp{1\{} \textit{CN} \asp{\}}$.
\end{enumerate}
\item By the inductive hypothesis it is the case that $M_P \models \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}, I\asp{)}$.
\item By the inductive hypothesis $M_P \models \asp{nifluent(}\textit{pro(}b, d\asp{)}, \textit{In}^{i})$.
\item By the inductive hypothesis it is the case that $M_P \models \asp{instant(}I\asp{)}$.
\end{enumerate}
Thus, we have shown assuming $S^{i}_{j} \models N^{\prime}$ then $\forall l \in B(r^{\prime}) : M_P \models l$, therefore $M_P \models \asp{holdsat(}n^{\prime}, \textit{In}^i, I \asp{)}$ and by construction of $S^{i}_{j}$ it is the case that $n^{\prime} \in S^{i}_{j}$.
\end{enumerate}
Therefore we have shown that if $\langle N, n \rangle \in \textit{DC}(S^{i}_{j})$ and $S^{i}_{j} \models N$ then $n \in \overline{\textit{DC}}^{i}(S^{i}_{j})$, consequently $n \in S^{i}_{j}$ and thus $\overline{\textit{DC}}^{i}(S^{i}_{j}) \subseteq S^{i}_{j}$.
\end{enumerate}
We have proven that $S^{i}_{j} = \overline{\textit{DC}}^{i}(S^{i}_{j})$.
\end{proof}

\subsection{Soundness Proof}
\label{proofSound}

\begin{proof}{\textbf{Theorem~\ref{theorSound} Soundness}} We need to show
\begin{enumerate}
\item According to \ref{eqIS1} $\forall i \in [1, n] : S^{i}_0 \subseteq \Delta^{i}$, $\exists \langle h, i \rangle \in R, n \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : n \in S^{h}_{0} \Rightarrow n \in S^{i}_{0}$, $\forall i \in [1,n] : S^{i}_0 = \textit{FD}^{i}(S^{i}_0)$ and $\forall i \in [1,n] : S^{i}_0 = \overline{\textit{DC}}^{i}(S^{i}_0)$.
\item According to Definition~\ref{defMLGModel} $\forall i \in [1, n], \forall j \in [1,k] : E^{i}_j = \textit{GR}^{i}(S^{i}_{j-1}, \{ \textit{se}^{i}_{j} \})$. Where $\textit{GR}^{i}$ is the event generation operation for an institution $\pazocal{I}^{i}$  w.r.t. $E = \langle E^{1}_{j}, ..., E^{n}_{j}\rangle$.
\item According to Definition~\ref{defMLGModel} $\forall i \in [1, n], \forall j \in [1,k+1] : S^{i}_j = \textit{TR}^{i}(S^{i}_{j-1}, E^{i}_{j})$. Where $\textit{TR}^{i}$ is the state transition operation for an institution $\pazocal{I}^{i}$  w.r.t. $S = \langle S^{1}_{j}, ..., S^{n}_{j}\rangle$.
\end{enumerate}
Each condition is dealt with separately:
\begin{enumerate}
\item $\forall i \in [1, n] : S^{i}_0 \subseteq \Delta^{i}$, $\exists \langle h, i \rangle \in R, n \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : n \in S^{h}_{0} \Rightarrow n \in S^{i}_{0}$, $\forall i \in [1,n] : S^{i}_0 = \textit{FD}^{i}(S^{i}_0)$ and $\forall i \in [1,n] : S^{i}_0 = \overline{\textit{DC}}^{i}(S^{i}_0)$:
\begin{enumerate}[label*=\arabic*.]
\item $\Delta^{i} \subseteq S^{i}_{0}$ - if $f \in \Delta^{i}$ then by \ref{eqASPMLTrans10} there is a rule with $r \in \Pi^{\pazocal{ML}(k)}$ such that $\asp{holdsat(}f, \textit{In}^{i}, I) \in H(r)$ and only one literal $\asp{start(I)} \in B(r)$ in the body, by \ref{eqASPSemTrans16} $\asp{start}(0) \in \Pi^{\pazocal{ML}(k)}$ is a fact and therefore $M_P \models \asp{holdsat(}f, \textit{In}^{i}, 0) $ and by construction of $S^{i}_{j}$ we have $f \in S^{i}_{0}$.
\item $\exists \langle h, i \rangle \in R, n \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : n \in S^{h}_{0} \Rightarrow n \in S^{i}_{0}$:
\begin{enumerate}[label*=\arabic*.]
\item According to \ref{eqASPMLTrans13} we have an AnsProlog rule \\$r = \asp{holdsat(} n \asp{, }\textit{In}^i \asp{, I) :- } \asp{holdsat(} n\asp{, }\textit{In}^h\asp{, I).}$
\item By 1.2.1. and construction of $S^{h}_{0}$ we have $M_P \models \asp{holdsat(} n\asp{, }\textit{In}^h\asp{, I)}$.
\item By \ref{eqASPSemTrans16} we have $\asp{instant(0)}. \in \Pi^{\pazocal{ML}(k)}$, a fact and therefore $M_P \models \asp{instant(0)}$ and thus $r$ is grounded s.t. $r = \asp{holdsat(} n \asp{, }\textit{In}^i \asp{, 0) :- }$ \\ $\asp{holdsat(} n\asp{, }\textit{In}^h\asp{, 0).} \in \Pi^{*}$.
\item By 1.2.2. and 1.2.3. $\forall l \in B(r^{\prime}) : M_P \models l$, therefore $M_P \models H(r^{\prime})$ and by construction of $S^{i}_{0}$ we have $f \in S^{i}_{0}$.
\end{enumerate}
We have shown $\exists \langle h, i \rangle \in R, n \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : n \in S^{h}_{0} \Rightarrow n \in S^{i}_{0}$.
\item $\forall i \in [1,n] : S^{i}_0 = \textit{FD}^{i}(S^{i}_0)$:
\begin{enumerate}
\item By \ref{eqDepFl1} and construction $S^{i}_0 \subseteq \textit{FD}^{i}(S^{i}_0)$.
\item By \ref{eqDepFl2} if $\exists X \in \pazocal{X}, f \in S^{i}_0, f^{\prime} \in \pazocal{D}^{i}(X, f) : S^{i}_0 \models X$ then $f^{\prime} \in S^{i}_0$.
\item By 1.3.ii and \ref{eqASPMLTrans12} we have an AnsProlog rule $r = \asp{holdsat(} f^{\prime}\asp{, }\textit{In}^i \asp{, I) :- } \\
\asp{holdsat(} f\asp{, }\textit{In}^i\asp{, I),} \; \textit{EX(X,} \pazocal{I}^i), \asp{instant(I).}$.
\item By  \ref{eqASPSemTrans16} we have $\asp{instant(0)}. \in \Pi^{\pazocal{ML}(k)}$, a fact and therefore $M_P \models \asp{instant(0)}$ and thus $r$ is grounded s.t. $r = \asp{holdsat(} f^{\prime}\asp{, }\textit{In}^i \asp{, 0) :- }$ \\ $\asp{holdsat(} f\asp{, }\textit{In}^i\asp{, 0),} \; \textit{EX(X,} \pazocal{I}^i), \asp{instant(0).} \in \Pi^{*}$.
\item By 1.3.iii and construction of $S^{i}_0$ we have $M_P \models \textit{EX(X,} \pazocal{I}^i)$ and $M_P \models \asp{holdsat(} f\asp{, }\textit{In}^i\asp{, I),}$.
\item By 1.3.iii, 1.3.iv and 1.3.v we have $\forall l \in B(r) : M_P \models l$, therefore $M_P \models H(r)$ and by construction of $S^{i}_{0}$ we have $f^{\prime} \in S^{i}_{0}$.
\end{enumerate}
By 1.3.i awe have $S^{i}_0 \subseteq \textit{FD}^{i}(S^{i}_0)$ and by 1.3.ii and 1.3.vi we have $ \textit{FD}^{i}(S^{i}_0) \subseteq S^{i}_0$, therefore we have shown $S^{i}_0 = \textit{FD}^{i}(S^{i}_0)$.
\item By Lemma~\ref{theoremAbstraction} we have $S^{i}_{0} = \overline{\textit{DC}}^{i}(S^{i}_{0})$.
\end{enumerate}
By 1.1. and 1.2. and 1.3. we have proven $\forall i \in [1, n] : S^{i}_0 \subseteq \Delta^{i}$, $\exists \langle h, i \rangle \in R, n \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : n \in S^{h}_{0} \Rightarrow n \in S^{i}_{0}$, $\forall i \in [1,n] : S^{i}_0 = \textit{FD}^{i}(S^{i}_0)$ and $\forall i \in [1,n] : S^{i}_0 = \overline{\textit{DC}}^{i}(S^{i}_0)$.
\item $\forall i \in [1, n], \forall j \in [k] : E^{i}_{j} = \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ - we prove by showing that $\textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \}) \subseteq E^{i}_{j}$ and $E^{i}_{j} \subseteq \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ separately.
\begin{enumerate}[label*=\arabic*.]
\item $\textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \}) \subseteq E^{i}_{j}$ - we will show that in Definition~\ref{defGR} all events \\ $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ according to \ref{eqGR10}-\ref{eqGR18} are in $E^{i}_{j}$ due to an applied rule $r \in \Pi^{\pazocal{ML}(k)}$ with $\asp{occurred(}e^{\prime}, \textit{In}^{i}, I\asp{)} \in H(r)$ and by construction of $E^{i}_{j}$.
\newcounter{grNeccProofCounter}
\begin{enumerate}[label*=\arabic*.]
\item According to \ref{eqGR10} $e^{\prime} = \textit{now}$ is necessarily in $\textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$. According \ref{eqASPMLTrans3} we have an AnsProlog rule $r \in \Pi^{\textit{base}(k)}$ and thus $r \in \Pi^{\pazocal{ML}(k)}$ s.t. $H(r) = \asp{occurred(}\textit{now}, \asp{In}, \asp{I)}$ and $B(r) = \{ \asp{instant(I)}, \asp{inst(In)}\}$. According to \ref{eqASPSemTrans16} we have facts $\asp{instant(j)} \in P^{*}$ and \ref{eqASPMLTrans1} $\asp{inst}(\textit{In}^{i}) \in P^{*}$. Thus we have $M_P \models \asp{occurred(}\textit{now}, \textit{In}^{i}, j\asp{)}$ and by construction of $E^{i}_{j}$, $\textit{now} \in E^{i}_{j}$.
\item According to \ref{eqGR11} $e^{\prime} \in \{ \textit{se}^{i}_{j} \}$ is necessarily in $\textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$, we will show $\textit{se}^{i}_{j} \in E^{i}_{j}$.
\begin{enumerate}[label*=\arabic*.]
\item By \ref{eqASPSemTrans10} we have a rule $r \in \Pi^{\pazocal{ML}(k)}$ such that \\$H(r) = \asp{observed(E, In, I)}$, by \ref{eqASPCompTraceTrans} we have a fact $\asp{observed(}e, j\asp{).} \in \Pi^{\pazocal{ML}(k)}$, by \ref{eqASPMLTrans1} $\asp{inst}(\textit{In}^{i}) \in \Pi^{\pazocal{ML}(k)}$ and therefore we have $M_P \models \asp{observed(}e, \textit{In}^{i}, j\asp{)}$.
\item According to Definition~\ref{defSynchTrace} either $\textit{se}^{i}_{j} \in \pazocal{E}^{i}_{\textit{obs}}$ or $\textit{se}^{i}_{j} = e_{\textit{null}}$.
\item If $\textit{se}^{i}_{j} \in \pazocal{E}^{i}_{\textit{obs}}$ then by \ref{eqASPMLTrans2} we have a fact $\asp{evtype(}e\asp{,} \textit{In}^{i}\asp{ex).} \in \Pi^{\pazocal{ML}(k)}$. By \ref{eqASPSemTrans4} we have a rule $r \in \Pi^{\pazocal{ML}(k)}$ such that $H(r) = \asp{occurred(E, In, I)}$ and the aforementioned literals modelled by $M_P$ we have \\$M_P \models \asp{occurred(}e, \textit{In}^{i}, j \asp{)}$ where $e \in \pazocal{E}^{i}$. 
\item If $\textit{se}^{i}_{j} = e_{\textit{null}}$ then by Definition~\ref{defSynchTrace} we know $e \not \in \pazocal{E}^{i}$, thus according to the translation in Definition~\ref{defASPMLTrans} we have $\asp{evtype(}e, \textit{In}^{i}, \asp{ex).} \not \in \Pi^{\pazocal{ML}(k)}$ and $\forall r \in \Pi^{*} : \asp{evtype(}e, \textit{In}^{i}, \asp{ex)} \neq H(r)$. Therefore $M_P \not \models \asp{evtype(}e, \textit{In}^{i}, \asp{ex)}$. Thus, we have by $\ref{eqASPSemTrans5}$ a rule $r \in \Pi^{\pazocal{ML}(k)}$ such that $H(r) = \asp{occurred(null, In, I)}$ where $\forall l \in B(r) : M_P \models l$ and the head is ground s.t. $M_P \models \asp{occurred(null,} \textit{In}^{i}, j\asp{)}$. 
\item By 3.1.2.3 and 3.1.2.4. and construction of $E^{i}_{j}$ we have $\textit{se}^{i}_{j} \in E^{i}_{j}$.
\end{enumerate}
\setcounter{grNeccProofCounter}{\theenumi}
\end{enumerate}
Conditions \ref{eqGR13}-\ref{eqGR17} depend recursively on an event already being in \\ $\textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ according to \ref{eqGR10} - \ref{eqGR18} or non-recursively depending on $S^{i}_{j} \models l$  for some literal $l$ in the case of \ref{eqGR14}-\ref{eqGR17}. We have already given the base cases for if according to \ref{eqGR10} - \ref{eqGR11} $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ then $e^{\prime} \in E^{i}_{j}$. We make the inductive hypothesis that $\forall i \in [1,n]$ if according to \ref{eqGR10}-\ref{eqGR18} $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ then $e^{\prime} \in E^{i}_{j}$. The inductive steps are given for \ref{eqGR13}-\ref{eqGR18} as follows:
\begin{enumerate}[label*=\arabic*.]
\setcounter{enumiii}{\thegrNeccProofCounter - 1}
\item \ref{eqGR13} -
\begin{enumerate}[label*=\arabic*.]
\item According to \ref{eqGR13} we have $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ if \\$X \in \pazocal{X}^{i} \wedge$ \\ $e \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \} \wedge S^{i}_{j} \models X \wedge e^{\prime} \in \pazocal{G}(X, e) \wedge S \models \textit{pow}(e^{\prime})$. 
\item By 2.1.3.1. and \ref{eqASPMLTrans9} we have a rule $r \in \Pi^{\pazocal{ML}(k)}$ such that $H(r) = \asp{occurred}(e^{\prime}, \textit{In}^{i}, \asp{I)}$. 
\item By 2.1.3.1. we have $S^{i}_{j} \models X$ and $S^{i}_{j} \models \textit{pow}(e^{\prime})$, and by the construction of $S^{i}_{j}$ we have $M_P \models \textit{EX(X,}\pazocal{I}^{i}\textit{)}$ and $M_P \models \asp{holdsat(pow(}e^{\prime}), \textit{In}^{i}, \asp{I)}$. 
\item By \ref{eqASPSemTrans16} we know we have a fact in $\Pi^{\pazocal{ML}(k)}$ such that \\$M_P \models \asp{instant(j)}$. 
\item By the inductive hypothesis we assume if $e \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ then $e \in E^{i}_{j}$, thus by construction of $E^{i}_{j}$ we have $M_P \models \asp{occurred}(e, \textit{In}^{i}, j\asp{)}$. 
\item By 2.1.3.2., 2.1.3.3., 2.1.3.4. and 2.1.3.5. all body literals of $r$ are true and therefore \\$M_P \models \asp{occurred}(e^{\prime}, \textit{In}^{i}, j\asp{)}$ and by construction of $E^{i}_{j}$ we have $e^{\prime} \in E^{i}_{j}$.
\end{enumerate}
\item \ref{eqGR14}-\ref{eqGR17} are dealt together due to their similarity 
\begin{enumerate}[label*=\arabic*.]
\item According to \ref{eqGR14}-\ref{eqGR17} $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ if $S^{i}_{j} \models f$ where $f = \textit{obl(a, d)}$ (\ref{eqGR14}, \ref{eqGR15}) or $f = \textit{pro(a, d)}$ (\ref{eqGR16}, \ref{eqGR17}), $e = \textit{disch(f)}$ (\ref{eqGR14}, \ref{eqGR16}) or $e = \textit{viol(f)}$ (\ref{eqGR15}, \ref{eqGR17}). 
\item The other conditions either depend on $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ for which by the inductive hypothesis we assume $e \in E^{i}_{j}$ and by construction of $E^{i}_{j}$, $M_P \models \asp{occurred}(e, \textit{In}^{i}, j\asp{)}$ 
\item Or, depend on some $f^{\prime} \in S^{i}_{j}$ for which we have by construction of  $S^{i}_{j}$, $M_P \models \asp{holdsat}(f^{\prime}, \textit{In}^{i}, j\asp{)}$. 
\item In the case of \ref{eqGR15} and \ref{eqGR17} the conditions also depend on $\textit{disch}(f) \not \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$, assuming that $E^{i}_{j} \subseteq \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ (subsequently proven) then if the conditions of \ref{eqGR15} or \ref{eqGR17} are met we have $\textit{disch}(f) \not \in E^{i}_{j}$ and by construction of $E^{i}_{j}$, $M_P \not \models \asp{occurred}(\asp{disch(}f\asp{),} \textit{In}^{i}, j\asp{)}$. 
\item According to \ref{eqASPSemTrans11} - \ref{eqASPSemTrans14} there is an AnsProlog rule $r \in \Pi^{\pazocal{ML}(k)}$ such that $H(r) = \asp{occurred}(e^{\prime}\asp{,} \textit{In}^{i}, j\asp{)}$.
\item By 2.1.3.1. to 2.1.3.5. all body literals of $r$ are true as and therefore $M_P \models \asp{occurred}(e^{\prime}\asp{,} \textit{In}^{i}, j\asp{)}$ and by construction of $E^{i}_{j}$ we have $e^{\prime} \in E^{i}_{j}$.
\end{enumerate}
\item \ref{eqGR18} -
\begin{enumerate}[label*=\arabic*.]
\item By \ref{eqASPMLTrans14} it is necessarily the case that  $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ if $\exists \langle h, i \rangle \in R, e^{\prime} \in \pazocal{E}^{h}_{\textit{norm}} \cap \pazocal{E}^{i}_{\textit{norm}}$.
\item By 2.1.4.1. and \ref{eqASPMLTrans14} we have all the conditions for an AnsProlog rule $r \in \Pi^{*}$ such that \\$H(r) = \asp{occurred}(e^{\prime}\asp{,} \textit{In}^{i}, j\asp{)}$ and $B(r) = \{ \asp{occurred(} e\asp{, }\textit{In}^h\asp{, I).} \}$. 
\item By the inductive hypothesis we assume for $h \in [1,n]$ that if \\$e \in \textit{GR}^{h}(S^{h}_{j}, \{ \textit{se}^{h}_{j} \})$ then $e \in E^{h}_{j}$. Hence, by 2.1.4.1. and construction of $E^{h}_{j}$ we have $M_P \models \asp{occurred(}e, \textit{In}^{h}, j \asp{)}$.ff
\item By 2.1.4.3. all body literals of $r$ are true and we have \\$M_P \models \asp{occurred}(e^{\prime}\asp{,} \textit{In}^{i}, j\asp{)}$.
\end{enumerate}
\end{enumerate}
We have proven $\textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \}) \subseteq E^{i}_{j}$.
\item $E^{i}_{j} \subseteq \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ - we will prove that if $e^{\prime} \in E^{i}_{j}$ then $e^{\prime}$ is one of the events described by the minimality constraints on $\textit{GR}^{i}$, \ref{eqGR1}-\ref{eqGR9}, and thus \\ $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$. We prove by showing that for each applied rule with $\asp{occurred(}e^{\prime}\asp{,}\textit{In}^{i}\asp{,} j\asp{)}$ in the head causes $e^{\prime} \in E^{i}_{j}$ such that $e^{\prime}$ is one of the literals in \ref{eqGR1}-\ref{eqGR9}. The relevant rules are \ref{eqASPSemTrans3}-\ref{eqASPSemTrans5} and \ref{eqASPSemTrans11}-\ref{eqASPSemTrans16}. For each of the rules being applied causing $e^{\prime} \in E^{i}_{j}$ we show $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$:
\begin{enumerate}[label*=\arabic*.]
\item \ref{eqASPSemTrans3} - by the construction of $E^{i}_{j}$, $e^{\prime} = \textit{now}$. According to \ref{eqGR1} $\textit{now} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\item \ref{eqASPSemTrans4} - 
\begin{enumerate}[label*=\arabic*.]
\item By \ref{eqASPSemTrans4} the body literals $M_P \models \asp{evtype(}e^{\prime}\asp{,} \textit{In}^{i} \asp{,ex} \asp{)}$ and \\ $M_P \models \asp{observed(}e^{\prime}\asp{,} \textit{In}^{i} \asp{,} j \asp{)}$, must be in the head of an applied rule in $\Pi^{\pazocal{ML}(k)}$. 
\item If $M_P \models \asp{evtype(}e^{\prime}\asp{,} \textit{In}^{i} \asp{,ex} \asp{)}$ then there must be a fact produced by \ref{eqASPMLTrans2} implying $e^{\prime} \in \pazocal{E}_{\textit{obs}}$. 
\item If $M_P \models \asp{observed(}e^{\prime}\asp{,} \textit{In}^{i} \asp{,} j \asp{)}$ then rule \ref{eqASPSemTrans10} is applied implying $M_P \models \asp{observed(}e^{\prime}\asp{,} j \asp{)}$.
\item By Definition~\ref{defASPCompTraceTrans} we have for the composite trace $\textit{ctr} = \langle e_0, ..., e_k \rangle$ a fact $\asp{observed(}e_j\asp{,} j \asp{).} \in \Pi^{\pazocal{ML}(k)}$. 
\item By 2.2.2.4. and \ref{defASPCompTraceTrans} $e^{\prime} = e_j$ or the rule \ref{eqASPSemTrans6} is applied such that $M_P \models \asp{observed(}e\asp{,} j \asp{)}$ where $e \neq e_j$ which would violate the constraint \ref{eqASPSemTrans7} and thus $M_P$ would not be an answer-set. 
\item By 2.2.2.5. and \ref{defASPCompTraceTrans} $\asp{observed(}e_j\asp{,} j \asp{).} \in \Pi^{\pazocal{ML}(k)}$,  $e^{\prime} = e_j$ and by 2.2.2.1. $M_P \models \asp{evtype(}e^{\prime}\asp{,} \textit{In}^{i} \asp{,ex} \asp{).} \in P$ and therefore by \ref{eqASPMLTrans2} $e_j \in \pazocal{E}^{i}$. 
\item Since $e_j \in \pazocal{E}^{i}$ we have by Definition~\ref{defSynchTrace} and 2.2.2.3. that $e^{\prime} = e_j = \textit{se}^{i}_{j}$.
\item According to \ref{eqGR2} $\textit{se}^{i}_{j} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\end{enumerate}
\item \ref{eqASPSemTrans5} - 
\begin{enumerate}[label*=\arabic*.]
\item By \ref{eqASPSemTrans5} and construction of $E^{i}_{j}$ we have $e^{\prime} = e_{\textit{null}}$, \\$M_P \not \models \asp{evtype(}e\asp{,} \textit{In}^{i} \asp{,ex} \asp{)}$ and $M_P \models \asp{observed(}e\asp{,} \textit{In}^{i} \asp{,} j \asp{)}$.
\item By 2.2.3.1. $M_P \not \models \asp{evtype(}e\asp{,} \textit{In}^{i} \asp{,ex} \asp{)}$ so \ref{eqASPMLTrans2} has not produced a fact implying $e \not \in \pazocal{E}_{\textit{obs}}$. 
\item By 2.2.3.1. $M_P \models \asp{observed(}e\asp{,} \textit{In}^{i} \asp{,} j \asp{)}$ then rule \ref{eqASPSemTrans10} is applied implying $M_P \models \asp{observed(}e\asp{,} j \asp{)}$. 
\item By Definition~\ref{defASPCompTraceTrans} we have for the composite trace $\textit{ctr} = \langle e_0, ..., e_k \rangle$ a fact $\asp{observed(}e_j\asp{,} j \asp{).} \in \Pi^{\pazocal{ML}(k)}$. Therefore, we either have by \ref{defASPCompTraceTrans} that $e = e_j$ or the rule \ref{eqASPSemTrans6} is applied such that $M_P \models \asp{observed(}e\asp{,} j \asp{)}$ where $e \neq e_j$ which would violate the constraint \ref{eqASPSemTrans7} and thus $M_P$ would not be an answer-set. Therefore $e = e_j$.
\item By \ref{defASPCompTraceTrans} we have that $\asp{observed(}e_j\asp{,} j \asp{).} \in \Pi^{\pazocal{ML}(k)}$, and $e = e_j$ and thus \\$M_P \not \models \asp{evtype(}e_j\asp{,} \textit{In}^{i} \asp{,ex} \asp{)}$. This implies by \ref{eqASPMLTrans2} that $e = e_j \not \in \pazocal{E}^{i}_{\textit{obs}}$, therefore according to Definition~\ref{defSynchTrace} given the synchronised trace $\textit{str} = \langle \textit{se}_0, ..., \textit{se}_k \rangle$ for $\pazocal{I}^{i}$ of $\textit{ctr}$ we have $\textit{se}_{j} = e_{\textit{null}}$. 
\item Since $e^{\prime} = e_{\textit{null}} = \textit{se}_{j}$ then according to \ref{eqGR2} $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\end{enumerate}
\item \ref{eqASPSemTrans11}-\ref{eqASPSemTrans14} - 
\begin{enumerate}[label*=\arabic*.]
\item By \ref{eqASPSemTrans11}-\ref{eqASPSemTrans14} and construction of $E^{i}_{j}$ we have $e^{\prime} = \textit{disch(f)}$ or $e^{\prime} = \textit{viol(f)}$ for some $f = \textit{obl(a, d)}$ or $f = \textit{pro(a, d)}$. 
\item According to \ref{eqASPSemTrans11}-\ref{eqASPSemTrans14} we have $M_P \models \asp{holdsat(}f\asp{,In,I)}$ and by construction of $S^{i}_{j}$, $S^{i}_{j} \models f$. 
\item Two rules, \ref{eqASPSemTrans12} and \ref{eqASPSemTrans14}, if applied depend on \\$M_P \not \models \asp{occurred(disch(}f\asp{)},In^{i},j\asp{)}$, by construction of $E^{i}_{j}$ we therefore have $\textit{disch(f)} \not \in E^{i}_{j}$.
\item By 3.1. $\textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \}) \subseteq E^{i}_{j}$ therefore if $e \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ then $e \in E^{i}_{j}$ and by contraposition if $\textit{disch(f)} \not \in E^{i}_{j}$ then $\textit{disch(f)} \not \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$. 
\item If one of \ref{eqASPSemTrans11}-\ref{eqASPSemTrans14} is applied then we either have \\$M_P \models \asp{holdsat(}p\asp{,In,I)}$ \\ or $M_P \models \asp{occurred(}p\asp{,}\textit{In}^{i}\asp{,}j\asp{)}$ where $p = a$ for \ref{eqASPSemTrans11} and \ref{eqASPSemTrans14} and $p = d$ for \ref{eqASPSemTrans12} and \ref{eqASPSemTrans13}. 
\item If we have $M_P \models \asp{holdsat(}p\asp{,In,I)}$ then the applied rule is a base case and by construction of $S^{i}_{j}$ we have $S^{i}_{j} \models p$.
\item If we have $M_P \models \asp{occurred(}p\asp{,In,I)}$ then the applied rule depends recursively on another applied rule, the base cases are \ref{eqASPSemTrans3}-\ref{eqASPSemTrans5} and \ref{eqASPSemTrans11}-\ref{eqASPSemTrans14} (which we prove separately).
\item If there is an applied rule $r \in \Pi^{\pazocal{ML}(k)}$ such that \\$H(r) = \asp{occurred(}e\asp{,}\textit{In}^{i}\asp{,}j\asp{)}$ for some $e$ then by construction of $E^{i}_{j}$ we have $e \in E^{i}_{j}$ we make the inductive hypothesis that $e \in  \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\item We give the inductive step for a rule $r$ \ref{eqASPSemTrans11} -\ref{eqASPSemTrans14} (other inductive steps are for \ref{eqASPMLTrans9} which we prove separately) where $H(r) = \textit{occurred(e, In, I)}$.  For \ref{eqASPSemTrans11} - \ref{eqASPSemTrans14} if $M_P \models \asp{occurred(}p\asp{,}\textit{In}^{i}\asp{,}j\asp{)}$ where $p = a$ for \ref{eqASPSemTrans11} and \ref{eqASPSemTrans14} and $p = d$ for \ref{eqASPSemTrans12} and \ref{eqASPSemTrans13} given that $p \in E^{i}_{j}$ then assume by the inductive hypothesis that $p \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$, therefore $e \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ 
\item By 2.2.4.4., 2.2.4.6. and 2.2.4.9. we have shown for each applied rule \ref{eqASPSemTrans11}-\ref{eqASPSemTrans14} such that if by construction $e \in E^{i}_{j}$ then we have the necessary conditions for $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\end{enumerate}
\item \ref{eqASPMLTrans9} - 
\begin{enumerate}[label*=\arabic*.]
\item If a rule $r$ generated by the transformation \ref{eqASPMLTrans9} is applied then we have $M_P \models \asp{occurred(} e^{\prime}\asp{, }\textit{In}^i \asp{,} j \asp{)}$ and by construction of $E^{i}_{j}$ we have $e^{\prime} \in E^{i}_{j}$. 
\item If $r$ is applied we  must also have $M_P \models \asp{holdsat(pow(}e^{\prime}\asp{),} \textit{In}^{i}\asp{, }j \asp{),}$ and $M_P \models \textit{EX(X,} \pazocal{I}^i)$, and by construction of $S^{i}_{j}$ that $S^{i}_{j} \models \asp{pow(}e^{\prime}\asp{),}$ and $S^{i}_{j} \models X$. 
\item If $r$ is applied then $M_P \models \asp{occurred(} e\asp{, }\textit{In}^i \asp{,} j \asp{)}$ which depends recursively on another applied rule. The base cases are \ref{eqASPSemTrans3}-\ref{eqASPSemTrans5} \ref{eqASPSemTrans11}-\ref{eqASPSemTrans14} (proven). If there is an applied rule $r \in \Pi^{\pazocal{ML}(k)}$ such that $H(r) = M_P \models \asp{occurred(}e\asp{,}\textit{In}^{i}\asp{,}j\asp{)}$ for some $e$ then by construction of $E^{i}_{j}$ we have $e \in E^{i}_{j}$. The inductive hypothesis is that $e \in  \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$. We assume by the inductive hypothesis that if \ref{eqASPMLTrans9} is applied then $M_P \models \asp{occurred(} e\asp{, }\textit{In}^i \asp{,} j \asp{)}$, by construction $e \in E^{i}_{j}$ and thus $e \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$. 
\item By 2.2.5.1. 2.2.5.2. and 2.2.5.3. and \ref{eqGR4} if $r$ is applied then $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\item Thus if a rule produced by \ref{eqASPMLTrans9} is applied then $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\end{enumerate}
\item \ref{eqASPMLTrans14} -
\begin{enumerate}[label*=\arabic*.]
\item If a rule $r$ generated by the transformation \ref{eqASPMLTrans14} is applied then we have $M_P \models \asp{occurred(} e^{\prime}\asp{, }\textit{In}^i \asp{,} j \asp{)}$ and by construction of $E^{i}_{j}$ we have $e^{\prime} \in E^{i}_{j}$. 
\item If $r$ is applied we  must also have for some $\langle h, i \rangle \in R, e \in \pazocal{E}^{h}_{\textit{norm}} \cap \pazocal{E}^{i}_{\textit{norm}}$
\item We also have that $M_P \models \asp{occurred(} e\asp{, }\textit{In}^h \asp{,} j \asp{)}$ which depends recursively on another applied rule. The base cases are \ref{eqASPSemTrans3}-\ref{eqASPSemTrans5} \ref{eqASPSemTrans11}-\ref{eqASPSemTrans14} (proven). The inductive hypothesis is that if there is an applied rule $r \in \Pi^{\pazocal{ML}(k)}$ such that $H(r) = \asp{occurred(}e\asp{,}\textit{In}^{h}\asp{,}j\asp{)}$ for some $e$, by construction of $E^{h}_{j}$ we have $e \in E^{h}_{j}$, then we have $e \in \textit{GR}^{h}(S^{h}_{j}, \{ \textit{se}^{h}_{j} \})$. We assume by the inductive hypothesis that if \ref{eqASPMLTrans14} is applied then $M_P \models \asp{occurred(} e\asp{, }\textit{In}^h \asp{,} j \asp{)}$, by construction $e \in E^{h}_{j}$ and thus \\$e \in \textit{GR}^{h}(S^{i}_{j}, \{ \textit{se}^{h}_{j} \})$.
\item Thus by 2.2.6.2., 2.2.6.3. and by \ref{eqGR9} $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$. 
\item Thus, if a rule produced by \ref{eqASPMLTrans14} is applied then $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\end{enumerate}
\end{enumerate}
We have proven that under the assumption that $e^{\prime} \in E^{i}_{j}$ then $e^{\prime} \in \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ and thus $E^{i}_{j} \subseteq \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\end{enumerate}
We have proven $E^{i}_{j} \subseteq \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$ and $\textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \}) \subseteq E^{i}_{j}$ therefore $E^{i}_{j} = \textit{GR}^{i}(S^{i}_{j}, \{ \textit{se}^{i}_{j} \})$.
\item $\forall i \in [1, n], \forall j \in [1,k] : S^{i}_j = \textit{TR}^{i}(S^{i}_{j-1}, E^{i}_{j})$ - by Definition~\ref{defST}:
\begin{enumerate}[label*=\arabic*.]
\item By definition~\ref{defST} We need to show that \\$f \in (S^{i}_{j} \cap \pazocal{F}^{i}_{\textit{inert}}) \backslash \textit{TERM}^{i}(S^{i}_{j}, E^{i}_{j}) \cup \textit{INIT}^{i}(S^{i}_{j}, E^{i}_{j})$ or $\exists \langle h, i \rangle \in R, f \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap$ \\ $ \pazocal{F}^{i}_{\textit{ninert}} : f \in S^{h}_{j}$ or $f \in \textit{FD}^{i}(S^{i}_j)$ or $f in \overline{\textit{DC}}^{i}(S^{i}_j)$ iff $f \in S^{i}_{j}$.
\item We will first show $f \in (S^{i}_{j} \cap \pazocal{F}^{i}_{\textit{inert}}) \backslash \textit{TERM}^{i}(S^{i}_{j}, E^{i}_{j}) \cup \textit{INIT}^{i}(S^{i}_{j}, E^{i}_{j})$ iff $f \in S^{i}_{j}$.
\begin{enumerate}[label*=\arabic*.]
\item We will show $f \not \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ iff \\$M_P \not \models \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$. We will show by contraposition $M_P \models \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ iff there is an applied rule $r \in P^{*}$ such that $H(r) = \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$. Therefore we will show a rule of the type \ref{eqASPMLTrans7} or \ref{eqASPSemTrans15} with $\asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ in the head is applied if and only if $f \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$.
\begin{enumerate}[label*=\arabic*.]
\item We will show \ref{eqASPMLTrans7} produces an applied rule $r$ such that $H(r) = \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ iff  we have all the conditions of \ref{eqFIT21}. The rule $r$ is applied such that $M_P \models  \asp{occurred(} e\asp{,} \textit{In}^i\asp{,} j-1 \asp{)}$, $M_P \models \textit{EX(X,} \pazocal{I}^i)$, $M_P \models \asp{holdsat(}f\asp{,} \textit{In}^{i}\asp{,} j-1 \asp{)}$, $M_P \models \asp{instant(}j-1\asp{)}$ iff $f \in \pazocal{C}^{i\downarrow}(X,e)$. Thus by construction we have $S^{i}_{j-1} \models X$, $S^{i}_{j-1} \models f$ and $e \in E^{i}_{j-1}$. Therefore a rule $r$ produced by the transformation \ref{eqASPMLTrans7} is applied iff  we have all the conditions of \ref{eqFIT21}.
\item We will show the rule $r$ in \ref{eqASPSemTrans15} is applied such that \\$H(r) = \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ iff we have all the conditions of \ref{eqFIT22}. The rule $r$ is applied such that $M_P \models \asp{occurred(viol}f\asp{),} \textit{In}^i\asp{,} j-1 \asp{)}$ or $M_P \models \asp{occurred(disch}f\asp{),} \textit{In}^i\asp{,} j-1 \asp{)}$, and $M_P \models \asp{holdsat(}f\asp{,} \textit{In}^{i}\asp{,} j-1 \asp{)}$. Thus $r$ is applied iff by construction we have $S^{i}_{j-1} \models X$, $S^{i}_{j-1} \models f$, and $\textit{disch}(f) \in E^{i}_{j-1}$ or $\textit{viol}(f) \in E^{i}_{j-1}$. Therefore the rule \ref{eqASPSemTrans15} is applied iff we have all the conditions of \ref{eqFIT22}.
\item Therefore a rule produced by \ref{eqASPMLTrans7} or the rule \ref{eqASPSemTrans15} is applied such that $H(r) = \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ iff \ref{eqFIT21} or \ref{eqFIT22} are met iff $f \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$.
\item By 3.1.1.1. - 3.1.1.3. a rule $r$ of type \ref{eqASPMLTrans7} or \ref{eqASPSemTrans15} is applied with $H(r) = \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j\asp{)}$ iff we have the conditions of \ref{eqFIT21} or \ref{eqFIT22} iff \\ $f \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$.
\end{enumerate}
By contraposition we have shown $\forall h \in [1,n] : f \not \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ iff \\$M_P \not \models \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$.
\item We will show that $f \in \textit{INIT}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ iff \\$M_P \models \asp{initiated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$. We have $M_P \models \asp{initiated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ iff there is an applied rule $r \in P^{*}$ such that $H(r) = \asp{initiated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ iff the rule $r$ is from the transformation \ref{eqASPMLTrans6}.
\begin{enumerate}[label*=\arabic*.]
\item We will show \ref{eqASPMLTrans6} produces an applied rule $r$ such that $H(r) = \asp{initiated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ iff we have all the conditions of \ref{eqFIT11}. According to \ref{eqASPMLTrans6} an applied rule $r$ is produced iff  $M_P \models \asp{occurred(} e\asp{, } \textit{In}^i \asp{,} j-1\asp{)}$ and $M_P \models \textit{EX(X,} \pazocal{I}^i)$ and $f \in \pazocal{C}^{i\uparrow}(X,e)$ iff by construction we have $e \in E^{i}_{j-1}$ and $S^{i}_{j-1} \models X$. Therefore the rule $r$ produced by the transformation \ref{eqASPMLTrans6} is applied iff we have all the conditions of \ref{eqFIT11} s.t. $f \in \textit{INIT}(S^{i}_{j-1}, E^{i}_{j-1})$.
\end{enumerate}
We have shown $f \in \textit{INIT}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ iff $M_P \models \asp{initiated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$.
\item We have shown $\forall h \in [1,n] : f \not \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ iff \\$M_P \not \models \asp{terminated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$ and \\ $f \in \textit{INIT}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ iff $M_P \models \asp{initiated(}f\asp{,}\textit{In}^{i}\asp{,}j-1\asp{)}$.
\item The rule $r$ in \ref{eqASPSemTrans1} where \\ $H(r) = \asp{holdsat(}f\asp{,} \textit{In}^{i}\asp{,} j \asp{)}$ such that\\$M_P \models \asp{ifluent(}f, \textit{In}^{i}\asp{)}$ iff \\$f \not \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ iff by construction $S^{i}_{j} \models f$ and \ref{eqASPMLTrans4} $f \in \pazocal{F}^{i}_{\textit{inert}}$.
\item By 3.2.1. the rule $r$ in \ref{eqASPSemTrans1} is applied iff \\$f \in S^{i}_{j-1} \cap \pazocal{F}^{i}_{\textit{inert}} \wedge f \not \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i})$ and therefore iff we have all the conditions in \ref{eqST11}.
\item By 3.2.2. the rule $r$ in \ref{eqASPSemTrans2} is applied where $H(r) = \asp{holdsat(}f\asp{,} \textit{In}^{i}\asp{,} j \asp{)}$, iff $M_P \models \asp{ifluent(}f, \textit{In}^{i}\asp{)}$, $f \in \textit{INIT}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ and $f \not \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i}_{j-1})$ iff $f \in \textit{INIT}^{i}(S^{i}_{j-1}, E^{i}) \wedge f \not \in \textit{TERM}^{i}(S^{i}_{j-1}, E^{i})$ and therefore iff we have all the conditions in \ref{eqST12}. 
\end{enumerate}
We have shown $f \in (S^{i}_{j} \cap \pazocal{F}^{i}_{\textit{inert}}) \backslash \textit{TERM}^{i}(S^{i}_{j}, E^{i}_{j}) \cup \textit{INIT}^{i}(S^{i}_{j}, E^{i}_{j})$ iff by construction $f \in S^{i}_{j}$.
\item We will now show $\exists \langle h, i \rangle \in R, n \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : n \in S^{h}_{0} \Rightarrow n \in S^{i}_{0}$ iff $f \in S^{i}_{j}$:
\begin{enumerate}[label*=\arabic*.]
\item According to \ref{eqASPMLTrans13} we have an AnsProlog rule \\$r = \asp{holdsat(} n \asp{, }\textit{In}^i \asp{, I) :- } \asp{holdsat(} n\asp{, }\textit{In}^h\asp{, I).}$
\item By 1.2.1. and construction of $S^{h}_{0}$ we have $M_P \models \asp{holdsat(} n\asp{, }\textit{In}^h\asp{, I)}$.
\item By \ref{eqASPSemTrans16} we have $\asp{instant(}j\asp{)}. \in \Pi^{\pazocal{ML}(k)}$, a fact and therefore $M_P \models \asp{instant(}j\asp{)}$ and thus $r$ is grounded s.t. \\$r = \asp{holdsat(} n \asp{, }\textit{In}^i \asp{, }j\asp{) :- }$ \\ $\asp{holdsat(} n\asp{, }\textit{In}^h\asp{, }j\asp{).} \in \Pi^{*}$.
\item By 3.3.2. and 3.3.3. $\forall l \in B(r^{\prime}) : M_P \models l$, therefore $M_P \models H(r^{\prime})$ and by construction of $S^{i}_{0}$ we have $f \in S^{i}_{j}$.
\end{enumerate}
We have shown $\exists \langle h, i \rangle \in R, n \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : n \in S^{h}_{0} \Rightarrow n \in S^{i}_{0}$ iff by construction $f \in S^{i}_{j}$.
\item We will now show $f \in \textit{FD}^{i}(S^{i}_{j})$ iff $f \in S^{i}_j$.
\begin{enumerate}
\item By \ref{eqDepFl1} and construction $S^{i}_j \subseteq \textit{FD}^{i}(S^{i}_j)$.
\item By \ref{eqDepFl2} if $\exists X \in \pazocal{X}, f \in S^{i}_j, f^{\prime} \in \pazocal{D}^{i}(X, f) : S^{i}_j \models X$ then $f^{\prime} \in S^{i}_j$.
\item By 3.4.ii and \ref{eqASPMLTrans12} we have an AnsProlog rule $r = \asp{holdsat(} f^{\prime}\asp{, }\textit{In}^i \asp{, I) :- } \\
\asp{holdsat(} f\asp{, }\textit{In}^i\asp{, I),} \; \textit{EX(X,} \pazocal{I}^i), \asp{instant(I).}$.
\item By  \ref{eqASPSemTrans16} we have $\asp{instant(}j\asp{)}. \in \Pi^{\pazocal{ML}(k)}$, a fact and therefore $M_P \models \asp{instant(}j\asp{)}$ and thus $r$ is grounded s.t. \\$r = \asp{holdsat(} f^{\prime}\asp{, }\textit{In}^i \asp{, }j\asp{) :- }$ \\ $\asp{holdsat(} f\asp{, }\textit{In}^i\asp{, }j\asp{),} \; \textit{EX(X,} \pazocal{I}^i), \asp{instant(}j\asp{).} \in \Pi^{*}$.
\item By 3.4.iii and construction of $S^{i}_j$ we have $M_P \models \textit{EX(X,} \pazocal{I}^i)$ and $M_P \models \asp{holdsat(} f\asp{, }\textit{In}^i\asp{, }j\asp{)}$.
\item By 3.4.iii, 3.4.iv and 3.4.v we have $\forall l \in B(r) : M_P \models l$, therefore $M_P \models H(r)$ and by construction of $S^{i}_{j}$ we have $f^{\prime} \in S^{i}_{j}$.
\end{enumerate}
We have shown $f \in \textit{FD}^{i}(S^{i}_{j})$ iff $f \in S^{i}_j$.
\item By Lemma~\ref{theoremAbstraction} we have $S^{i}_{0} = \overline{\textit{DC}}^{i}(S^{i}_{0})$.
\item By 3.2., 3.3., 3.4. and 3.5. we have proven $f \in (S^{i}_{j} \cap \pazocal{F}^{i}_{\textit{inert}}) \backslash \textit{TERM}^{i}(S^{i}_{j}, E^{i}_{j}) \cup \textit{INIT}^{i}(S^{i}_{j}, E^{i}_{j})$ or $\exists \langle h, i \rangle \in R, f \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : f \in S^{h}_{j}$ or $f \in \textit{FD}^{i}(S^{i}_j)$ or $f in \overline{\textit{DC}}^{i}(S^{i}_j)$ iff $f \in S^{i}_{j}$. 
\end{enumerate}
We have proven $\forall i \in [1, n], \forall j \in [1,k] : S^{i}_j = \textit{TR}^{i}(S^{i}_{j-1}, E^{i}_{j})$.
\end{enumerate}
We have proven a) $\forall i \in [1, n] : S^{i}_0 \subseteq \Delta^{i}$, $\exists \langle h, i \rangle \in R, n \in (\pazocal{F}^{h}_{\textit{cnorm}} \cup \pazocal{F}^{h}_{\textit{anorm}}) \cap \pazocal{F}^{i}_{\textit{ninert}} : n \in S^{h}_{0} \Rightarrow n \in S^{i}_{0}$, $\forall i \in [1,n] : S^{i}_0 = \textit{FD}^{i}(S^{i}_0)$ and $\forall i \in [1,n] : S^{i}_0 = \overline{\textit{DC}}^{i}(S^{i}_0)$. b) $\forall i \in [1, n], \forall j \in [1,k] : E^{i}_j = \textit{GR}^{i}(S^{i}_{j-1}, \{ \textit{se}^{i}_{j} \})$. Where $\textit{GR}^{i}$ is the event generation operation for an institution $\pazocal{I}^{i}$  w.r.t. $E = \langle E^{1}_{j}, ..., E^{n}_{j}\rangle$. c) $\forall i \in [1, n], \forall j \in [1,k+1] : S^{i}_j = \textit{TR}^{i}(S^{i}_{j-1}, E^{i}_{j})$. Where $\textit{TR}^{i}$ is the state transition operation for an institution $\pazocal{I}^{i}$  w.r.t. $S = \langle S^{1}_{j}, ..., S^{n}_{j}\rangle$. Therefore we have proven $M$ is the model of $\pazocal{ML}$ w.r.t. $\textit{ctr}$.
\end{proof}

\subsection{Completeness Proof} 
\label{proofCompl}

To prove completeness we take the same approach as in \cite[p. 161]{Cliffe2007}.

\begin{proof}{\textbf{Theorem~\ref{theorCompl} Completeness}} We need to show that $M_P$ is a model for $P^{*}$ and also a \textit{minimal} model for $P^{*}$. We show the interpretation $M_P$ is a model for the reduct of $P^{*, M_P}$ of $P^{*}$ w.r.t $M_P$. Let $r \in P^{*, M_P}$ be an applicable rule. We need to show that $M_P \models \textit{H}(r)$, that the rule is applied. Each type of rule from Definition~\ref{defASPMLTrans}, Definition~\ref{defASPDCATrans}, Definition~\ref{defASPCompTraceTrans} and Definition~\ref{defASPMLSemTrans} is addressed.
\begin{itemize}
\item \textit{r} is a fact of type \ref{eqASPMLTrans1}-\ref{eqASPMLTrans5} or a fact in \ref{eqASPSemTrans16}. True by construction of $M_P$.
\item \textit{r} is of type \ref{eqASPSemTrans1} -  by the reduct we know $\asp{terminated(}f, \textit{In}^{i}, j\asp{)}$ is false. By \ref{eqThCo4} for $f$ at $j$ we know $f \in S^{i}_{j}$ and by \ref{eqThCo1} $M_P \models \asp{holdsat(}f, \textit{In}^{i}, j\asp{)}$.
\item \textit{r} is of type \ref{eqASPSemTrans2} -  $\asp{initiated(}f, \textit{In}^{i}, j\asp{)}$ since $f \in S^{i}_{j}$ and $f \not \in S^{i}_{j-1}$ by \ref{eqThCo3}. By \ref{eqThCo3} and \ref{eqThCo1} $M_P \models \asp{holdsat(}f, \textit{In}^{i}, j\asp{)}$.
\item \textit{r} is of type \ref{eqASPSemTrans3} - from the way $\asp{instant(}j)$ is created in \ref{eqThCo13} we can infer that $\exists j \in [k] : E^{i}_{j}$. From \ref{eqGR10} and \ref{eqThCo6} we infer $M_P \models \asp{occurred(now}, \textit{In}^{i}, j)$.
\item \textit{r} is of type \ref{eqASPSemTrans4} - we know $\asp{observed}(e_{\textit{obs}}, \textit{In}^{i}, j)$ atoms originate from the composite trace \textit{ctr}. Given that $M_P \models \asp{evtype}(e_{\textit{obs}}, \textit{In}^{i}, \asp{ex})$ by \ref{eqThCo9} we have $e_\textit{obs} \in \pazocal{E}^{i}_{\textit{obs}}$ and by \ref{defSynchTrace} we have a synchronised trace $\textit{str}^{i} = \langle e_0, ..., e_k \rangle $ for $\pazocal{I}^{i}$ where $e_j = e_{\textit{obs}}$. Therefore by the definition of a multi-level governance institution model \ref{defMLGModel} and by \ref{eqGR11} we know $e_{\textit{obs}} \in E^{i}_{j}$. Therefore by \ref{eqThCo6} $M_P \models \asp{occurred}(e_{\textit{obs}}, \textit{In}^{i}, j)$.
\item \textit{r} is of type \ref{eqASPSemTrans5} - we know $\asp{observed}(e_{\textit{obs}}, \textit{In}^{i}, j)$ atoms originate from the composite trace \textit{ctr}. By the reduct we know $\asp{evtype}(e_{\textit{obs}}, \textit{In}^{i}, \asp{ex})$ is not true, this implies by \ref{eqThCo9} $e_\textit{obs} \not \in \pazocal{E}^{i}_{\textit{obs}}$ and by \ref{defSynchTrace} we have a synchronised trace $\textit{str}^{i} = \langle e_0, ..., e_k \rangle $ for $\pazocal{I}^{i}$ where $e_j = e_{\textit{null}}$. Therefore by \ref{eqThCo7} we have $M_P \models \asp{occurred}(\asp{null}, \textit{In}^{i}, j)$.
\item \textit{r} is of type \ref{eqASPSemTrans6} - always true.
\item \textit{r} is of type \ref{eqASPSemTrans7} - true by structure of \textit{ctr} and \ref{eqThCo5}.
\item \textit{r} is of type \ref{eqASPSemTrans8}, \ref{eqASPSemTrans9} or \ref{eqASPSemTrans10} - true by \ref{eqThCo5}.
\item \textit{r} is of type \ref{eqASPSemTrans11} or \ref{eqASPSemTrans13} - by construction this implies $e \in E^{i}_{j}$ or $e \in S^{i}_{j}$, and by \ref{eqASPSemTrans11} $\textit{obl}(e, d) \in S^{i}_{j}$ or by \ref{eqASPSemTrans13}  $\textit{pro}(a, e) \in S^{i}_{j}$. Therefore by \ref{eqGR14} or \ref{eqGR16} we have $\textit{disch}(\textit{obl}(e, d)) \in E^{i}_{j}$ or $\textit{disch}(\textit{pro}(a, e)) \in E^{i}_{j}$ and thus $M_P \models H(r)$.
\item \textit{r} is of type \ref{eqASPSemTrans12} or \ref{eqASPSemTrans14} - similar to the previous case, by construction this implies $e \in E^{i}_{j}$ or $e \in S^{i}_{j}$, and by \ref{eqASPSemTrans12} $\textit{obl}(a, e) \in S^{i}_{j}$ or by \ref{eqASPSemTrans14}  $\textit{pro}(e, d) \in S^{i}_{j}$. By the reduct and construction of $E^{i}_{j}$ we know $\textit{disch}(\textit{obl}(e, d)) \not \in E^{i}_{j}$ by \ref{eqASPSemTrans12} or $\textit{disch}(\textit{pro}(a, e)) \in E^{i}_{j}$ by \ref{eqASPSemTrans14}. Therefore by \ref{eqGR15} or \ref{eqGR17} we have $\textit{viol}(\textit{obl}(a, e)) \in E^{i}_{j}$ or $\textit{viol}(\textit{pro}(e, d)) \in E^{i}_{j}$ and thus $M_P \models H(r)$.
\item \textit{r} is of type \ref{eqASPSemTrans15} - by construction we know $N \in S^{i}_{j}$ and $\textit{disch}(N) \in E^{i}_{j}$ or $\textit{viol}(N) \in E^{i}_{j}$ and by \ref{eqASPMLTrans4} $N \in \pazocal{F}^{i}_{\textit{inert}}$. Therefore we have the conditions for $N \in S^{i}_{j} \backslash S^{i}_{j+1} \cap \pazocal{F}^{i}_{\textit{inert}}$ by \ref{eqFIT22}, \ref{eqST11} or \ref{eqST12}, and \ref{eqMLGM4}. Thus by \ref{eqThCo4} we have $M_P \models H(r)$.
\item \textit{r} is of type \ref{eqASPSemTrans16} where $H(r)$ is a \asp{next/2} atom - $M_P \models H(r)$ by \ref{eqThCo13} and \ref{eqThCo15}.
\item \textit{r} is of type \ref{eqASPMLTrans6} - from the creation of the rule and the fact that the body elements are true we infer $f \in \pazocal{F}^{i}_{\textit{inert}}$ and by \ref{eqThCo1} $S^{i}_{j} \models X$, by \ref{eqThCo6} that $e \in E^{i}_{j}$ and $f \in \pazocal{C}^{\i \uparrow}(X, e)$. By $M$ being a model and by \ref{eqFIT11} we have the conditions for $f \in \textit{INIT}(S^{i}_{j}, E^{i}_{j})$. By the reduct we know $S^{i}_{j-1} \not \models f$ and by \ref{eqMLGM4}, \ref{eqST12} we have $S^{i}_{j} \models f$. Therefore we have all the conditions for $M_P \models H(r)$ by \ref{eqThCo3}.
\item \textit{r} is of type \ref{eqASPMLTrans7} - from the creation of the rule and the fact that the body elements are true we infer $f \in \pazocal{F}^{i}_{\textit{inert}}$ and by \ref{eqThCo1} $S^{i}_{j} \models X$ and $S^{i}_{j} \models f$, by \ref{eqThCo6} that $e \in E^{i}_{j}$ and $f \in \pazocal{C}^{i \downarrow}(X, e)$. By $M$ being a model and by \ref{eqFIT11} we have the conditions for $f \in \textit{TERM}(S^{i}_{j}, E^{i}_{j})$. By \ref{eqMLGM4} and \ref{eqST11} we have $S^{i}_{j + 1} \not \models f$. Therefore we have all the conditions for $M_P \models H(r)$ by \ref{eqThCo4}.
\item \textit{r} is of type \ref{eqASPMLTrans9} - from the creation of the rule and the fact that the body elements are true we infer $S^{i}_{j} \models X$, $S^{i}_{j} \models \textit{pow}(e^{\prime})$, $e \in E^{i}_{j}$  and $e^{\prime} \in \pazocal{G}^{i}(X, e)$. By $M$ being a model and by \ref{eqGR13}  we have the conditions for $e^{\prime} \in E^{i}_{j}$. Therefore we have all the conditions for $M_P \models H(r)$ by \ref{eqThCo2}.
\item \textit{r} is of type \ref{eqASPMLTrans12} - from the creation of the rule and $\pazocal{D}^{i}$ in definition~\ref{def:inst} we infer that $f^{\prime} \in \pazocal{F}^{i}_{\textit{ninert}}$, $S^{i}_{j} \models X$ and $S^{i}_{j} \models f$. We have all the conditions such that by $M$ being a model and \ref{eqDepFl2} we conclude $M_P \models H(r)$ by \ref{eqThCo1}.
\item \textit{r} is of type \ref{eqASPMLTrans10} - from the creation of the rule we infer $f \in \Delta^{i}$. By Definition~\ref{defMLGModel} and \ref{eqIS1} and since $\overline{\textit{DC}}^{i}$ is monotonic we infer that $f \in S^{i}_{0}$. Therefore by \ref{eqThCo14} and \ref{eqThCo1} we have $M_P \models H(r)$.
\item \textit{r} is of type \ref{eqASPMLTrans13} - from the creation of the rule we infer that $f^{\prime} \in \pazocal{F}^{i}_{\textit{ninert}}$ and $\langle h, i \rangle \in R$. By the rule being applied we infer that $S^{h}_{j} \models f$ and $S^{i}_{j} \models f$. We have all the conditions such that by $M$ being a model and \ref{eqST13} we conclude $M_P \models H(r)$.
\item \textit{r} is of type \ref{eqASPMLTrans14} - from the creation of the rule we infer that $e^{\prime} \in \pazocal{E}^{i}_{\textit{norm}}$ and $\langle h, i \rangle \in R$. By the rule being applied we infer that $e \in E^{h}_{j}$ and $e \in E^{i}_{j}$. We have all the conditions such that by $M$ being a model and \ref{eqGR18} we conclude $M_P \models H(r)$.
\item \textit{r} is of type \ref{eqASPMLTrans11} - from the creation of the rule this implies $f \equiv f^{\prime}$, by Definition\ref{defStateForm} $S^{i}_{j} \models f$ and by \ref{eqThCo1} $M_P \models H(r)$.
\item \textit{r} is of type \ref{eqASPDCATrans1}, \ref{eqASPDCATrans2}, \ref{eqASPDCATrans5}, \ref{eqASPDCATrans6}, \ref{eqASPDCATrans3}, \ref{eqASPDCATrans4}, - we will first show by induction that for a rule $r^{\prime}$ of these types such that $r^{\prime} = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-}$ \\ $\textit{CN}, C, \asp{nifluent(}n^{\prime}, \textit{In}^{i} \asp{),} \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \asp{instant(I).}$, if $\exists \textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN} : M_P \models \textit{EX}(X, \pazocal{I}^{i})$  then $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$. We will then show that the rule $r$ being applied means that $n^{\prime} \in \overline{\textit{DC}}^{i}(S^{i}_{j})$ and consequently $M_P \models H(r)$.
\begin{enumerate}[label*=\arabic*.]
\item First, by induction on two counters:
\begin{enumerate}[label*=\arabic*.]
\item \textbf{Base case 1:} \ref{eqASPDCATrans1} and \ref{eqASPDCATrans5} -
\begin{enumerate}[label*=\arabic*.]
\item The transformations \ref{eqASPDCATrans1} and \ref{eqASPDCATrans5} gives $r^{\prime} = \asp{holdsat}(n, \textit{In}^{i}, j) \asp{:-}$ \\ $\textit{CN}, C, \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \\ \asp{nifluent(}n, \textit{In}^{i} \asp{),} \asp{instant(I).}$ or \\$r^{\prime} = \asp{holdsat}(n, \textit{In}^{i}, j) \asp{:-} \textit{CN}, C,\asp{nifluent(}n, \textit{In}^{i} \asp{),} \asp{instant(I).}$ such that $n \in \pazocal{F}^{i}_{\textit{anorm}}$.
\item If $\exists \textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN} : M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then by construction of $S^{i}_{j}$ we know that $S^{i}_{j} \models X$ and if $M_P \models \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j)$ then $S^{i}_{j} \models \textit{pow}(a)$.
\item By the creation of $r^{\prime}$ we have $b \in \pazocal{G}^{i}(X, a) \cup \pazocal{D}^{i}(X, a)$ and $a \in \pazocal{E}^{i}_{\textit{inst}} \cup \pazocal{F}^{i}$.
\item Therefore by 1.1.1, 1.1.2, 1.1.3 if $\textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}, M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then we have all the conditions of \ref{eqDC1} for $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$.
\end{enumerate}
\item \textbf{Base case 2:} \ref{eqASPDCATrans2} -
\begin{enumerate}[label*=\arabic*.]
\item The transformations \ref{eqASPDCATrans2} and \ref{eqASPDCATrans6} give us $r^{\prime} = \asp{holdsat}(n, \textit{In}^{i}, j) \asp{:-}$ \\ $\textit{CN}, C, \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \\ \asp{nifluent(}n, \textit{In}^{i} \asp{),} \asp{instant(I).}$ or \\$r^{\prime} = \asp{holdsat}(n, \textit{In}^{i}, j) \asp{:-} \textit{CN}, C, \asp{nifluent(}n, \textit{In}^{i} \asp{),} \\ \asp{instant(I).}$ such that $n \in \pazocal{F}^{i}_{\textit{anorm}}$. 
\item If $\exists \textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN} : M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then by construction of $S^{i}_{j}$ we know that $S^{i}_{j} \models X$ and if $M_P \models \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j)$ then $S^{i}_{j} \models \textit{pow}(a)$.
\item By the creation of $r^{\prime}$ we have $b \in \pazocal{G}^{i}(X, a) \cup \pazocal{D}^{i}(X, a)$ and $a \in \pazocal{E}^{i}_{\textit{inst}} \cup \pazocal{F}^{i}$. \item Therefore by 1.2.1, 1.2.2 and 1.2.3 if $\textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}, M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then we have all the conditions of \ref{eqDC2} for $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$.
\end{enumerate}
\item \textbf{Inductive hypothesis:} - A rule $r^{\prime}$ is of type \ref{eqASPDCATrans1}, \ref{eqASPDCATrans2}, \ref{eqASPDCATrans5}, \ref{eqASPDCATrans6}, \ref{eqASPDCATrans3}, \ref{eqASPDCATrans4} such that $r^{\prime} = \\ \asp{holdsat}(n, \textit{In}^{i}, j) \asp{:-} \textit{CN}, C, \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \asp{nifluent(}n, \textit{In}^{i} \asp{),} \asp{instant(I).}$ or \\$r^{\prime} =\asp{holdsat}(n, \textit{In}^{i}, j) \asp{:-} \textit{CN}, C, \asp{nifluent(}n, \textit{In}^{i} \asp{),} \asp{instant(I).}$, and $n \in \pazocal{F}^{i}_{\textit{anorm}}$. If $\textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN} : M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$.
\item \textbf{Inductive step 1:} \ref{eqASPDCATrans3} -
\begin{enumerate}[label*=\arabic*.]
\item The transformation \ref{eqASPDCATrans3} gives us $r^{\prime \prime} = \asp{holdsat}(\textit{obl}(n^{\prime}, d), \textit{In}^{i}, j) \asp{:-}$ \\ $\textit{CN}^{\prime \prime}, C^{\prime \prime}, \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j),$ \\ $\asp{nifluent(}\textit{obl}(n^{\prime}, d), \textit{In}^{i} \asp{),}$ \\ $\asp{instant(I).}$ or \\$r^{\prime \prime} = \asp{holdsat}(\textit{obl}(n^{\prime}, d), \textit{In}^{i}, j) \asp{:-} \textit{CN}^{\prime \prime}, C^{\prime \prime}, \asp{nifluent(}\textit{obl}(n^{\prime}, d), \textit{In}^{i}\asp{),} \asp{instant(I).}$ where \\$\textit{obl}(n^{\prime}, d) \in \pazocal{F}^{i}_{\textit{anorm}}$.
\item We know that $r^{\prime \prime}$ is created conditional on a rule \\$r^{\prime} = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-}$ \\ $\textit{CN}^{\prime}, C^{\prime}, \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \asp{nifluent(}n^{\prime}, \textit{In}^{i} \asp{),} \asp{instant(I).}$ or \\$r^{\prime} = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-} \textit{CN}^{\prime}, C^{\prime}, \asp{nifluent(}n^{\prime}, \textit{In}^{i} \asp{),} \asp{instant(I).}$. 
\item By the inductive hypothesis if $\textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime}, M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$. 
\item By the creation of $r^{\prime \prime}$ and 3 we know that $\textit{CN}^{\prime \prime}$ is constructed such that $\textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime}, M_P \models \textit{EX}(X, \pazocal{I}^{i})$ iff $\textit{EX(obl(n, d)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime \prime}, M_P \models \textit{EX}(X, \pazocal{I}^{i})$. 
\item If $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ then by \ref{eqDC1} $\langle N^{\prime}, \textit{obl}(n^{\prime}, d) \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$ iff $\textit{obl}(n, d) \in N^{\prime}$.
\item By 1.4.3, 1.4.4 and 1.4.5 if $\textit{EX}(\textit{obl}(n, d)) \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime \prime},$ \\ $M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then $\langle N^{\prime}, \textit{obl}(n^{\prime}, d) \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $\textit{obl}(n^{\prime}, d) \in N^{\prime}$.
\end{enumerate}
\item \textbf{Inductive step 2:} \ref{eqASPDCATrans4} -
\begin{enumerate}[label*=\arabic*.]
\item The transformation \ref{eqASPDCATrans4} gives us $r^{\prime \prime} = \asp{holdsat}(\textit{pro}(n^{\prime}, d), \textit{In}^{i}, j) \asp{:-} \\ \textit{CN}^{\prime \prime}, C^{\prime \prime}, \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \asp{nifluent(}\textit{pro}(n^{\prime}, d), \textit{In}^{i}\asp{),} \asp{instant(I).}$ or \\ $r^{\prime \prime} = \asp{holdsat}(\textit{pro}(n^{\prime}, d), \textit{In}^{i}, j) \asp{:-} \\ \textit{CN}^{\prime \prime}, C^{\prime \prime}, \asp{nifluent(}\textit{pro}(n^{\prime}, d), \textit{In}^{i}\asp{),} \asp{instant(I).}$ where $\textit{pro}(n^{\prime}, d) \in \pazocal{F}^{i}_{\textit{anorm}}$.
\item We know that $r^{\prime \prime}$ is created conditional on rules of the form \\$r^{\prime} = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-}$ \\ $\textit{CN}^{\prime}, C^{\prime},$ \\ $\asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \asp{nifluent(}n^{\prime}, \textit{In}^{i} \asp{),} \asp{instant(I).}$ or \\$r^{\prime} = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-} \textit{CN}^{\prime}, C^{\prime}, \asp{nifluent(}n^{\prime}, \textit{In}^{i} \asp{),} \asp{instant(I).}$.
\item By the inductive hypothesis for all rules $r^{\prime}$ if $\textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime}, M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$. 
\item By the creation of $r^{\prime \prime}$ and 3 we know that $\textit{CN}^{\prime \prime}$ is constructed such that for all rules $r^{\prime}$ we have \\$\textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime}, M_P \models \textit{EX}(X, \pazocal{I}^{i})$ iff $\textit{EX(pro(n, d)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime \prime}, M_P \models \textit{EX}(X, \pazocal{I}^{i})$.
\item For all rules $r^{\prime}$ if $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ then by \ref{eqDC2} we have that $\langle N^{\prime}, \textit{pro}(n^{\prime}, d) \rangle \in$ \\ $\textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$ iff $\textit{pro}(n, d) \in N^{\prime}$.
\item By 1.5.3, 1.5.4 and 1.5.5 if $\textit{EX}(\textit{pro}(n, d)) \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN}^{\prime \prime}$ if $M_P \models \textit{EX}(X, \pazocal{I}^{i})$ then $\langle N^{\prime}, \textit{pro}(n^{\prime}, d) \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $\textit{pro}(n, d) \in N^{\prime}$.
\end{enumerate}
We have shown by induction that a rule $r^{\prime}$ of type \ref{eqASPDCATrans1}, \ref{eqASPDCATrans2}, \ref{eqASPDCATrans5}, \ref{eqASPDCATrans6}, \ref{eqASPDCATrans3} or \ref{eqASPDCATrans4} such that \\$r^{\prime} = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-} \textit{CN}, C, \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \asp{instant(I).}$ or \\$r^{\prime} = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-} \textit{CN}, C, \asp{instant(I).}$, if $\exists \textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN} : M_P \models \textit{EX}(X, \pazocal{I}^{i})$  then $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$.
\end{enumerate}
\item We will now show if $r$ of type \ref{eqASPDCATrans1}, \ref{eqASPDCATrans2}, \ref{eqASPDCATrans5}, \ref{eqASPDCATrans6}, \ref{eqASPDCATrans3} or \ref{eqASPDCATrans4} is applied then $n^{\prime} \in \overline{\textit{DC}}^{i}(S^{i}_{j})$ and consequently $M_P \models H(r)$:
\begin{enumerate}[label*=\arabic*.]
\item If $r$ is of type \ref{eqASPDCATrans1}, \ref{eqASPDCATrans2}, \ref{eqASPDCATrans5}, \ref{eqASPDCATrans6} \ref{eqASPDCATrans3} or \ref{eqASPDCATrans4} then \\$r = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-} \textit{CN}, C, \asp{holdsat}(\textit{pow}(b), \textit{In}^{i}, j), \asp{instant(I).}$ or \\$r = \asp{holdsat}(n^{\prime}, \textit{In}^{i}, j) \asp{:-} \textit{CN}, C,\asp{instant(I).}$.
\item Under the semantics of aggregates if $r$ is applied then $C$ must be true and $\exists \textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN} : M_P \models \textit{EX}(X, \pazocal{I}^{i})$.
\item By 1 we have for all $\textit{EX(n)} \asp{:} \textit{EX}(X, \pazocal{I}^{i})\asp{;} \in \textit{CN} : M_P \models \textit{EX}(X, \pazocal{I}^{i})$  then $\langle N, n^{\prime} \rangle \in \textit{DC}^{i}(S^{i}_{j})$ such that $n \in N$.
\item Since $r$ is applied we know that $\textit{CN}$ is true, therefore by 2.3. and construction in \ref{eqThCo1} iff $S^{i}_{j} \models N$. Therefore we have $\langle N, n^{\prime} \rangle \in \overline{\textit{DC}}^{i}(S^{i}_{j})$. such that $\forall n \in N : S^{i}_{j} \models n$
\item By Definition~\ref{defDC} we have $n \in \overline{\textit{DC}}^{i}(S^{i}_{j})$, by \ref{eqMLGM2} and \ref{eqIS4} for $j=0$ or \ref{eqMLGM4} and \ref{eqST15} $j \neq 0$ we have $S^{i}_{j} \models n^{\prime}$ and by construction $M_P \models H(r)$.
\end{enumerate}
\end{enumerate}
\end{itemize}
We have shown for every applicable rule $r \in P^{*, M_P}$ that $M_P \models H(r)$ and thus $M_P$ is a model of $P^{*, M_P}$. We will now show that $M_P$ is a \textit{minimal} model of $P^{*, M_P}$ by proving there does not exist a model of $P^{*, M_P}$ that is a strict subset of $M_P$. Let the program $P^{*, M_P \prime}$ be the program comprising all applied rules in $P^{*, M_P}$ stratified into levels $\pi_x$ according to:
\begin{itemize}[label={}]
\item \ref{eqASPMLTrans1} - $\asp{inst(}\textit{In}^i\asp{)} : \pi_0 .$
\item \ref{eqASPMLTrans2} - $\asp{evtype(e,} \textit{In}^i \asp{,ex)} : \pi_0 .$
\item \ref{eqASPMLTrans3} - $\asp{evtype(e,} \textit{In}^i \asp{,inst)} : \pi_0 .$
\item \ref{eqASPMLTrans4} - $\asp{ifluent(f, }\textit{In}^i\asp{)} : \pi_0.$
\item \ref{eqASPMLTrans5} - $\asp{nifluent(f, }\textit{In}^i\asp{)} : \pi_0 .$
\item $\begin{aligned} \text{\ref{eqASPMLTrans6} -} \asp{initiated(} p\asp{, } \textit{In}^i \asp{, J)}: \pi_{3J+2} \asp{:- } & \asp{occurred(} e\asp{, } \textit{In}^i \asp{,} I\asp{)} : \pi_{3J+1}, \\ & \asp{not} \; \asp{holdsat(}p, \textit{In}^{i}, \asp{J)} : \pi_{3J}, \\ &
\textit{EX(X,} \pazocal{I}^J) : \pi_{3J}, \\ \asp{instant(J)} : \pi_0.\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPMLTrans7} -} \asp{terminated(} p\asp{, }\textit{In}^i \asp{, J)}: \pi_{3J+2} \asp{:- } & \asp{occurred(} e\asp{,} \textit{In}^i\asp{, J)} : \pi_{3J+1}, \\ & 
\textit{EX(X,} \pazocal{I}^i) : \pi_{3J}, \\ & \asp{holdsat(}f\asp{,} \textit{In}^{i}\asp{, J)} : \pi_{3J}, \asp{instant(J)} : \pi_{0}.\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPMLTrans9} - } \asp{occurred(} e^{\prime}\asp{, }\textit{In}^i \asp{, J)} : \pi_{3J+1} \asp{:- } & \asp{occurred(} e\asp{, }\textit{In}^i\asp{, J)}: \pi_{3J+1}, \asp{holdsat(pow(}e^{\prime}\asp{),} \textit{In}^{i}\asp{, J)} : \pi_{3J}\asp{,} \\ & \textit{EX(X,} \pazocal{I}^i) : \pi_{3J}, \asp{instant(J)} : \pi_{0}. \end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPMLTrans12} - } \asp{holdsat(} f^{\prime}\asp{, }\textit{In}^i \asp{, J) :- } \; \; \asp{holdsat(} f\asp{, }\textit{In}^i\asp{, J),} \; \textit{EX(X,} \pazocal{I}^i), \asp{instant(J).} : \pi_{3J} \end{aligned}$
\item $\text{\ref{eqASPMLTrans10} -} \asp{holdsat(} f\asp{, } \textit{In}^i, \asp{J)} : \pi_{3J} \asp{:-} \asp{start(J)} : \pi_{0} \asp{.}$
\item $\begin{aligned} \text{\ref{eqASPMLTrans13} - } \asp{holdsat(} n \asp{, }\textit{In}^i \asp{, J)} : \pi_{3J} \asp{:-} \asp{holdsat(} n\asp{, }\textit{In}^h\asp{, J).} : \pi_{3J} \end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPMLTrans14} - } \asp{occurred(} e \asp{, }\textit{In}^i \asp{, I)} : \pi_{3J+1} \asp {:- }  \asp{occurred(} e\asp{, }\textit{In}^h\asp{, I).} : \pi_{3J+1} \end{aligned}$
\item $\text{\ref{eqASPMLTrans11} - }\asp{holdsat(} \textit{f}\asp{, } \textit{In}^i, \asp{J)} : \pi_{J} :- \asp{holdsat(} \textit{f}^{\prime}\asp{, } \textit{In}^i, \asp{J)} : \pi_{J} \asp{, } \asp{instant(J)} : \pi_{0}.$
\item $\text{\ref{eqASPDCATrans1} - } \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i \asp{,J)} : \pi_{3J} \asp{ :- } \textit{CN} : \pi_{3J} \asp{,} C : \pi_{3J} \asp{,}\asp{holdsat(pow(}b\asp{),} \textit{In}^{i}\asp{, I)} : \pi_{3J}, \asp{nifluent(obl(}b, d)\asp{, }\textit{In}^i\asp{)} : \pi_0, \\ \asp{instant(I)} : \pi_{0} \asp{.}$
\item $\text{\ref{eqASPDCATrans2} - } \asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i \asp{,I)} : \pi_{3J} \asp{ :- }$ \\ $\textit{CN}\asp{,} : \pi_{3J} \textit{C} : \pi_{3J} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}\asp{, I)} : \pi_{3J},$ \\ $\asp{nifluent(pro(}b, d)\asp{, } : \pi_0, \\ \asp{instant(J)} : \pi_{0} \asp{.}$
\item $\text{\ref{eqASPDCATrans5} - } \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i \asp{,J)} : \pi_{3J} \asp{ :- } \textit{CN} : \pi_{3J} \asp{,} C : \pi_{3J}, \asp{nifluent(obl(}b, d)\asp{, }\textit{In}^i\asp{)} : \pi_0, \\ \asp{instant(I)} : \pi_{0} \asp{.}$
\item $\text{\ref{eqASPDCATrans6} - } \asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i \asp{,I)} : \pi_{3J} \asp{ :- } \textit{CN}\asp{,} : \pi_{3J} \textit{C} : \pi_{3J} \asp{,} \\ \asp{instant(J)} : \pi_{0} \asp{.}$
\item $\text{\ref{eqASPDCATrans3} - } \asp{holdsat(obl(}b, d\asp{)}, \textit{In}^i \asp{,I)} : \pi_{3J} \asp{ :- } \textit{CN}, : \pi_{3J} C  : \pi_{3J} \asp{,} \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}\asp{, I)} : \pi_{3J}, \asp{nifluent(obl(}b, d)\asp{, } \textit{In}^{i} \asp{),}  : \pi_{0}, \asp{instant(I).} : \pi_{0}$
\item $\begin{aligned} \text{\ref{eqASPDCATrans4} - } \asp{holdsat(pro(}b, d\asp{)}, \textit{In}^i \asp{,I)} : \pi_{3J} \asp{ :- } & \textit{CN}, C : \pi_{3J}, \\ & \asp{holdsat(pow(}b\asp{),} \textit{In}^{i}\asp{, I)} : \pi_{3J}, \\ & \asp{nifluent(obl(}b, d)\asp{, } \textit{In}^{i} \asp{),}  : \pi_{0}, \\ & \asp{instant(I).} : \pi_{0} \end{aligned}$
\item $\text{\ref{eqASPCompTraceTrans} -} \asp{observed(\textit{e}_{\textit{i}}, J).} : \pi_{0}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans1} -}
\asp{holdsat(P,In,J)} : \pi_{3J} \asp{:-} & \asp{holdsat(P,In,J)} : \pi_{3J}, \asp{not \; terminated(P,In,H)} : \pi_{3H+2}, \\ &  \asp{next(H,J)} : \pi_{0}  \asp{,} \\ & \asp{ifluent(P, In).} : \pi_{0} \end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans2} -}
\asp{holdsat(P,In,J)} : \pi_{3J} \asp{:-} & \asp{initiated(P,In,J)} : \pi_{3J+2}, \\ &
	\asp{next(I,J)} : \pi_{0}, \\ &
    \asp{ifluent(P, In)} : \pi_{0}.
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans3} -}
\asp{occurred(now, In, J)} : \pi_{3J+1} \asp{:- instant(J)} : \pi_{0}, \asp{inst(In)} : \pi_{0}.
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans4} -}
\asp{occurred(E,In,J)} : \pi_{3J+1} \asp{:- evtype(E,In,ex)} : \pi_{0} \asp{,observed(E,In,J)}: \pi_{3J}.
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans5} -}
\asp{occurred(null,In,J)} : \pi_{3J+1} \asp{:- not\; evtype(E,In,ex)} : \pi_{0}, \asp{observed(E,In,J)} : \pi_{3J}.
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans6} -} \asp{\{observed(E, J)\}} : \pi_{3J} \asp{:-} & \asp{evtype(E,In,ex)} : \pi_{0}, \asp{instant(J)} : \pi_{0}, \asp{not\; final(J)} : \pi_{0}, \\ & \asp{inst(In)} : \pi_{0}. \end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans7} -} 
\asp{ :- } & \asp{observed(E,J)} : \pi_{3J},\asp{observed(F,J)} : \pi_{3J}, \asp{instant(J)} : \pi_{0}, \\ & \asp{evtype(E,InX,ex)} : \pi_{0}, \\ & \asp{evtype(F,InY,ex)} : \pi_{0}, E!=F : \pi_{0}, \asp{inst(InX;InY)} : \pi_{0}.
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans8} -} \asp{obs(J)} : \pi_{3J} \asp{:-} & \asp{observed(E,J)} : \pi_{3J},\asp{evtype(E,In,ex)} : \pi_{0}.
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans9} -}
\asp{ :- not\; obs(J)} : \pi_{3J}, not\; \asp{final(J)} : \pi_{0}, \asp{instant(J)} : \pi_{0}.
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans10} -}
\asp{observed(E,In,J)} : \pi_{3J} :- \asp{observed(E,J)} : \pi_{3J}, \asp{inst(In)} : \pi_{0}.
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans11} -}
\asp{occurred(disch(obl(A, D)),In,J)} : \pi_{3J+1} \asp{:-} & \asp{holdsat(obl(A, D),In,J)} : \pi_{3J} , \\
& \asp{1\{occurred(A,In,J)} : \pi_{3J+1}, \\ & \asp{holdsat(A, In, J)} : \pi_{3J} \asp{\}.}
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans12} -} \asp{occurred(viol(obl(a, d))},\textit{In}^{i}, \asp{J)} : \pi_{3J+1} \asp{:-} & \asp{holdsat(obl(a, d)},\textit{In}^{i}, \asp{J)} : \pi_{3J} \asp{,} \\ & \asp{not\;} \\ & \asp{occurred(} \\ & \asp{disch(obl(a, d))}, \textit{In}^{i}, \asp{J)} : \pi_{3J+1} \asp{,} \\ & 
\asp{1\{occurred(d},\textit{In}^{i}, \asp{J)} : \pi_{3J+1} \asp{,} \\ & 
\asp{holdsat(d,} \textit{In}^{i}, \asp{J)\} } : \pi_{3J} \asp{.} \end{aligned}$.
\item $\begin{aligned}\text{\ref{eqASPSemTrans13} -}\asp{occurred(disch(pro(A, D)),In,J)} : \pi_{3J+1} \asp{:-} & \asp{
   holdsat(pro(A, D),In,J)} : \pi_{3J}, \\ & 
   \asp{1\{occurred(D,In,J),} : \pi_{3J+1} \\ & \asp{holdsat(D, In, J)} : \pi_{3J} \asp{\}.} \end{aligned}$
\item $\begin{aligned}\text{\ref{eqASPSemTrans14} -}
\asp{occurred(viol(pro(A, D)),In,J)} : \pi_{3J+1} \asp{:-} & \asp{holdsat(pro(A, D)),In,J)}: \pi_{3J} \asp{,} \\ & \asp{1\{occurred(A,In,J)} : \pi_{3J+1} \asp{,} \\ & 
\asp{holdsat(A, In, J)} : \pi_{3J} \asp{\}}, \\ & \asp{not\; occurred(} \\ & \asp{disch(pro(A, D)), In, J)} : \pi_{3J+1}.\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans15} -}
\asp{terminated(N,In,J)} : \pi_{3J+2} \asp{:-} &
   \asp{1\{occurred(viol(N),In,J)} : \pi_{3J+1}, \\ & \asp{occurred(disch(N),In,J)} : \pi_{3J+1} \asp{\}}, \\& \asp{ifluent(N,In)} : \pi_{0}, \asp{holdsat(N,In,J) : \pi_{3J}.}
\end{aligned}$
\item $\begin{aligned} \text{\ref{eqASPSemTrans16} -} & \asp{final(\textit{k})} : \pi_{0} .\; \\ &
 \asp{start(0)} : \pi_{0}. \; \asp{instant(0..T) : \pi_{0} :- final(T)}: \pi_{0}.  \; \\ &
 \asp{next(T, T+1)} : \pi_{0} \asp{:- instant(T)} : \pi_{0} . \end{aligned}$
% Note for future in case needed: Initially I was going to prove that we do not have a cyclic dependency graph by the fact that M_P is a model (in the formal framework). However, since we are only dealing with applied rules this is not necessary. We also do not need to prove that P is in general stratisfied (which isn't true). Since there is not always a unique answer-set, there is no answer-set if there is no model in the formal framework due to an ontological inconsistency.
\end{itemize}
Now we will show $M_P$ is a minimal model. Let $Z$ be an interpretation such that $Z \subset M_P$. Let $l$ be the lowest strata in which $Z$ and $M_P$ differ in atoms for $P^{*, M_P, \prime}$. Let $S$ be the set of atoms $s \in S$ such that $s : \pi_l$ is stratified at strata $l$ and $s \in M_P \backslash Z$. For an $s \in S$ we show it must be the head of an applied rule in $P^{*, M_P \prime}$.
\begin{enumerate}[label*=\arabic*.]
\item $s$ is a fact, then $Z$ cannot be a model of $P^{*, M_P \prime}$ since one of \ref{eqASPMLTrans1}-\ref{eqASPMLTrans5} or a fact in \ref{eqASPSemTrans16} is not applied.
\item $s = \asp{holdsat(}f^{\prime}, \textit{In}^{i}, j)$ -
\begin{enumerate}[label*=\arabic*.]
\item By $M_P \models s$ and construction we have $S^{i}_{j} \models f^{\prime}$, therefore either:
\begin{enumerate}[label*=\arabic*.]
\item by Definition~\ref{defStateForm} and construction of $M_P$: $M_P \models \asp{holdsat}(f, \textit{In}^{i}, j)$ for a rule $r$ created by \ref{eqASPMLTrans11}, or
\item by Definition~\ref{eqIS1} \ref{eqIS2} and construction of $M_P$: $M_P \models \asp{holdsat}(f, \textit{In}^{i}, j)$ for a rule $r$ created by \ref{eqASPMLTrans10}, or
\item by Definition~\ref{defDC} and construction of $M_P$: $M_P \models \textit{EX}(X, \pazocal{I}^{i})$, in the case of \ref{eqDCCl2} $M_P \models \asp{holdsat}(\textit{pow}(b, \textit{In}^{i}, j)$ and $M_P \models \textit{EX}(N, \pazocal{I}^{i})$ for a rule $r$ created by \ref{eqASPDCATrans1}, \ref{eqASPDCATrans2}, \ref{eqASPDCATrans5}, \ref{eqASPDCATrans6}, \ref{eqASPDCATrans3}, \ref{eqASPDCATrans4}, or 
\item by Definition~\ref{defST} or by Definition~\ref{defInitialStates} and construction of $M_P$: $M_P \models \textit{EX}(X, \pazocal{I}^{i})$ and $M_P \models \textit{EX}(X, \pazocal{I}^{i})$ and $M_P \models \asp{holdsat}(g, \textit{In}^{i}, j)$ for a rule $r$ created by \ref{eqASPMLTrans13}, or
\item by \ref{eqST11} $M_P \models \asp{holdsat}(f, \textit{In}^{i}, j-1)$ for the rule $r$ \ref{eqASPSemTrans1}, or 
\item by \ref{eqST12} and construction of $M_P$: $M_P \models \asp{initiated}(f, \textit{In}^{i}, j)$ for the rule $r$ \ref{eqASPSemTrans2}.
\end{enumerate}
For each possible $r$ the atoms true in the body of the rule are of a lower strata to $s$ and therefore must be in $Z$. Thus, one of the rules is applicable but not applied. Thus $Z$ cannot be a model.
\end{enumerate}
\item $s = \asp{occurred}(e, \textit{In}^{i}, j)$ - by construction $M_P \models s$ means that $e \in E^{i}_{j}$, implying $e \in \pazocal{E}^{i}$. We deal separately with each type of event in $\pazocal{E}$:
\begin{enumerate}[label*=\arabic*.]
\item $e \in \pazocal{E}^{i}_{\textit{obs}}$ - by construction of $M_P$ this implies $\asp{observed}(e, j). \in P^{*}$, a fact, therefore either $Z \not \models \asp{observed}(e, j)$ and $Z$ is not a model, or $Z \models \asp{observed}(e, j)$ meaning \ref{eqASPSemTrans4} is applied and thus for $Z$ to be a model we must have $Z \models \asp{occurred}(e, \textit{In}^{i}, j)$ but we do not and thus $Z$ is not a model.
\item $e \in \pazocal{E}^{i}_{\textit{inst}}$ - by construction of $M_P$ this implies either condition \ref{eqGR13} or \ref{eqGR18} for $e \in E^{i}_{j}$ are true. Respectively, we must have a rule $r \in P^{*}$ of type \ref{eqASPMLTrans9} or \ref{eqASPMLTrans14} such that $H(r) = \asp{occurred}(e, \textit{In}^{i}, j)$. The rule $r$ has body literals of a lower strata than $s$ thus they must be modelled by $Z$, this means $r$ is applied and therefore since $Z \not \models s$ thus $Z$ is not a model.
\item $e = e_{\textit{null}}$ - by \ref{eqThCo7} this implies $e_{\textit{null}} = \textit{str}^{i}_{j}$ therefore by the definition of a synchronised trace, Definition~\ref{defSynchTrace}, we have a composite event trace $\langle \textit{ctr}_0, ..., \textit{ctr}_{k} \rangle$ such that $\textit{ctr}_j \not \in \pazocal{E}_{\textit{obs}}$. This implies we do not have a fact $\asp{evtype}(\textit{ctr}_j, \textit{In}^{i}, \asp{ex)}. \in P^{*}$ by \ref{eqASPMLTrans2}. Therefore, by the reduct we have an applicable rule $r \in P^{*}$ of the type \ref{eqASPSemTrans5} such that $H(r) = \asp{occurred(null}\textit{In}^{i}, j \asp{)}$. However, since $Z \not \models \asp{occurred(null}\textit{In}^{i}, j \asp{)}$ then $r$ is not applied, meaning $Z$ is not a model.
\item $e \in \pazocal{E}^{i}_{\textit{norm}}$ - this implies the conditions of one of \ref{eqGR14}, \ref{eqGR15}, \ref{eqGR16} must be true \ref{eqGR17}. Thus, by construction of $E^{i}_{j}$ and $S^{i}_{j}$ we have the conditions for a rule $r$ of type \ref{eqASPSemTrans11}, \ref{eqASPSemTrans12}, \ref{eqASPSemTrans13} or \ref{eqASPSemTrans14} such that $H(r) = \asp{occurred}(e, \textit{In}^{i}, j)$. Since by the reduct negated elements of $B(r)$ are removed, all remaining elements of $B(r)$ are of a lower strata than $s$ therefore all body elements of $r$ are true and thus $r$ is an applicable rule. However, since $Z \not \models \asp{occurred}(e, \textit{In}^{i}, j)$ we know $r$ is not applied and therefore $Z$ is not a model.
\end{enumerate}
\item $s = \asp{initiated}(f, \textit{In}^{i}, j)$ - by \ref{eqThCo4} we know that $f \in S^{i}_{j}$, $f \not \in S^{i}_{j-1}$ and $f \in \pazocal{F}^{i}_{\textit{inert}}$. Since $M$ is a model this means we must have by Definition~\ref{defIndFlInTe} $f \in \textit{INIT}(S^{i}_{j}, E^{i}_{j})$:
\begin{enumerate}[label*=\arabic*.]
\item Condition \ref{eqFIT11} - thus we have $S^{i}_{j} \models f$, $f \in \pazocal{C}^{i \uparrow}(X, e)$, $S^{i}_{j} \models X$ and $e \in E^{i}_{j}$. By the creation of $E^{i}_{j}$ and $S^{i}_{j}$ this means we have all the conditions for an applicable rule $r \in P^{*}$ of type \ref{eqASPMLTrans6} such that $H(r) = s$ and all the body literals are true in $M_P$. Since all the body literals are of a lower strata than $s$ we conclude they are also true in $Z$, therefore $r$ is an applicable rule but since $Z \not \models s$ it is not applied and therefore $Z$ is not a model.
\end{enumerate}
\item $s = \asp{terminated}(f, \textit{In}^{i}, j)$ - by \ref{eqThCo4} we know that $f \in S^{i}_{j}$, $f \not \in S^{i}_{j+1}$ and $f \in \pazocal{F}^{i}_{\textit{inert}}$. Since $M$ is a model this means we must have by Definition~\ref{defIndFlInTe} $f \in \textit{TERM}(S^{i}_{j}, E^{i}_{j})$. We deal with each of the conditions required for $f$ to be in one of these sets:
\begin{enumerate}[label*=\arabic*.]
\item Condition \ref{eqFIT21} - thus we have $S^{i}_{j} \models f$, $f \in \pazocal{C}^{i \downarrow}(X, e)$, $S^{i}_{j} \models X$ and $e \in E^{i}_{j}$. By the creation of $E^{i}_{j}$ and $S^{i}_{j}$ this means we have all the conditions for an applicable rule $r \in P^{*}$ of type \ref{eqASPMLTrans7} such that $H(r) = s$ and all the body literals are true in $M_P$. Since all the body literals are of a lower strata than $s$ we conclude they are also true in $Z$, therefore $r$ is an applicable rule but since $Z \not \models s$ it is not applied and therefore $Z$ is not a model.
\item Condition \ref{eqFIT22} - thus we have $S^{i}_{j} \models f$, and $\textit{viol}(f) \in E^{i}_{j}$ or $\textit{disch}(f) \in E^{i}_{j}$. Since $f \in \pazocal{F}^{i}_{\textit{inert}}$ we have by \ref{eqASPMLTrans4} $\asp{ifluent}(f, \textit{In}^{i})\asp{.} \in P^{*}$ is a fact. By the creation of $E^{i}_{j}$ and $S^{i}_{j}$ this means we have all the conditions for an applicable rule $r \in P^{*}$ of type \ref{eqASPSemTrans15} such that $H(r) = s$ and all the body literals are true in $M_P$. Since all the body literals are of a lower strata than $s$ we conclude they are also true in $Z$, therefore $r$ is an applicable rule but since $Z \not \models s$ it is not applied and therefore $Z$ is not a model.
\end{enumerate}
\item $s = \asp{next}(j, j+1)$ - by \ref{eqThCo15} this implies $j < k$ thus by the rule $\ref{eqASPSemTrans16}$ with the $\asp{instant/3}$ atom in the head we have $M_P \models \asp{instant(}j)$. Thus we have an applicable rule $r \in P^{*}$ where $H(r) = \asp{next}(j, j+1)$ of type at \ref{eqASPSemTrans16} with a body atom that is true in $M_P$. Since the body comprises only an $\asp{instant/3}$ atom of a lower strata than $s$ it is also true in $Z$. But since $Z \not \models s$ it is not applied and therefore $Z$ is not a model.
\end{enumerate}
Therefore, we have shown for all possible cases that $Z$ cannot be a model if it is a strict subset of $M_P$ differing on strata $i$. Thus, $M_P$ is a \textit{minimal model} of $P^{*,M_P}$ and therefore an answer-set for $P^{*}$.
\end{proof}

==> chapter-2-background/Images/deonsq.tex <==
\begin{tikzpicture}
\draw[very thick, >=latex,->] (-4,3) -- (-4,1.4);
\draw[very thick] (-4,1.4) -- (-4,0);
\draw[very thick, >=latex,->] (-1,3) -- (-1,1.4);
\draw[very thick] (-1,1.4) -- (-1,0);
\draw[very thick, color=black!30!green, ->>] (-2.4,0) -- (-1,0);
\draw[very thick, color=black!30!green, <<-] (-4,0) -- (-2.4,0);
\draw[very thick, color=blue, dashed] (-4,3) -- (-1,3);

\draw[very thick, color=black!10!red, dotted] (-4,0) -- (-1,3);
\draw[very thick, color=black!10!red, dotted] (-4,3) -- (-1,0);
\node at (-4.2,3.4) {Obligatory $\textbf{O}p$};
\node at (-0.8,3.4) {Prohibited $\textbf{F}p$};
\node at (-4.2,-0.4) {Permissible $\textbf{P}p$};
\node at (-0.8,-0.4) {Omissible $\textbf{P}\neg p$};
\end{tikzpicture}

==> chapter-2-background/Images/deonsq.tex.preview__tud14072_s_conflicted_copy_2016-03-08_.tex <==
%& C:\Users\thomas\AppData\Roaming\TikzEdt\TikzEdt\023~1.0\TEMP_H~1
\begin{document}
\begin{tikzpicture}
\draw[very thick, >=latex,->] (-4,3) -- (-4,1.4);
\draw[very thick] (-4,1.4) -- (-4,0);
\draw[very thick, >=latex,->] (-1,3) -- (-1,1.4);
\draw[very thick] (-1,1.4) -- (-1,0);
\draw[very thick, color=black!30!green, ->>] (-2.4,0) -- (-1,0);
\draw[very thick, color=black!30!green, <<-] (-4,0) -- (-2.4,0);
\draw[very thick, color=blue, dashed] (-4,3) -- (-1,3);

\draw[very thick, color=black!10!red, dotted] (-4,0) -- (-1,3);
\draw[very thick, color=black!10!red, dotted] (-4,3) -- (-1,0);
\node at (-4.2,3.4) {Obligatory $\textbf{O}p$};
\node at (-0.8,3.4) {Prohibited $\textbf{F}p$};
\node at (-4.2,-0.4) {Permissible $\textbf{P}p$};
\node at (-0.8,-0.4) {Omissible $\textbf{P}\neg p$};

\usetikzlibrary{calc}
\pgftransformreset
\node[inner sep=0pt,outer sep=0pt,minimum size=0pt,line width=0pt,text width=0pt,text height=0pt] at (current bounding box) {};
%add border to avoid cropping by pdflibnet
\foreach \border in {0.1}
  \useasboundingbox (current bounding box.south west)+(-\border,-\border) rectangle (current bounding box.north east)+(\border,\border);
\newwrite\metadatafile
\immediate\openout\metadatafile=\jobname_BB.txt
\path
  let
    \p1=(current bounding box.south west),
    \p2=(current bounding box.north east)
  in
  node[inner sep=0pt,outer sep=0pt,minimum size=0pt,line width=0pt,text width=0pt,text height=0pt,draw=white] at (current bounding box) {
\immediate\write\metadatafile{\p1,\p2}
};
\immediate\closeout\metadatafile
\end{tikzpicture}

\end{document}





{document}

ent}







}
ment}







closeout\metadatafile
\end{tikzpicture}

\end{document}


}

\end{document}



==> chapter-2-background/Images/highlevelmlg.tex <==
\begin{tikzpicture}
\node at (-16.8,1.8) {\parbox{20mm}{\color{blue}Increasingly Abstract Regulations}};
\draw[very thick, color=blue, >=latex,->] (-15.6,-1) -- (-15.6,4.8);

\draw [rounded corners=1pt] (-8.8,5.2) rectangle (-5.8,4.2) node[pos=.5] {\textbf{Institution}};
\draw[very thick, dashed] (-12.2,3.6) -- (-8.8,4.2);
\node at (-7.2,3.8) {Governs};
\draw[very thick, dashed] (-2.2,3.6) -- (-5.8,4.2);

\fill (-7.2,3.2) circle (1mm);
\fill (-7.2,2.8) circle (1mm);
\fill (-7.2,2.4) circle (1mm);

\fill[rounded corners=1pt, black!10!red] (-12.2,2) rectangle (-9.2,1) node[pos=.5] {\parbox{30mm}{\centering \color{white}{\textbf{Non-compliant Institution}}}};
\fill[rounded corners=1pt, black!30!green] (-8.6,2) rectangle (-5.6,1) node[pos=.5] {\parbox{30mm}{\centering \color{white}{\textbf{Compliant Institution}}}};
\fill[rounded corners=1pt, black!30!green] (-5,2) rectangle (-2,1) node[pos=.5] {\parbox{30mm}{\centering \color{white}{\textbf{Compliant Institution}}}};

\draw[very thick, dashed] (-14,-0.2) -- (-12.2,1);
\node at (-10.6,0.4) {Governs};
\draw[very thick, dashed] (-7.4,-0.2) -- (-9.2,1);

\draw[very thick, dashed] (-10.4,-0.2) -- (-8.6,1);
\node at (-7,0.4) {Governs};
\draw[very thick, dashed] (-3.8,-0.2) -- (-5.6,1);

\draw[very thick, dashed] (-3.2,-0.2) -- (-5,1);
\node at (-2.6,0.4) {Governs};
\draw[very thick, dashed] (-0.2,-0.2) -- (-2,1);

\fill[rounded corners=1pt, black!30!green] (-14,-0.2) rectangle (-11,-1.2) node[pos=.5] {\parbox{30mm}{\centering \color{white}{\textbf{Compliant Institution}}}};
\fill[rounded corners=1pt, black!30!green] (-10.4,-0.2) rectangle (-7.4,-1.2) node[pos=.5] {\parbox{30mm}{\centering \color{white}{\textbf{Compliant Institution}}}};
\fill[rounded corners=1pt, black!10!red] (-6.8,-0.2) rectangle (-3.8,-1.2) node[pos=.5] {\parbox{30mm}{\centering \color{white}{\textbf{Non-compliant Institution}}}};
\fill[rounded corners=1pt, black!30!green] (-3.2,-0.2) rectangle (-0.2,-1.2) node[pos=.5] {\parbox{30mm}{\centering \color{white}{\textbf{Compliant Institution}}}};

\draw[very thick, dashed] (-15,-2.8) -- (-14,-1.2);
\node at (-12.8,-1.8) {Governs};
\draw[very thick, dashed] (-11.8,-2.8) -- (-11,-1.2);
\draw[very thick, dashed] (-11.8,-2.8) -- (-10.4,-1.2);
\node at (-8.6,-1.8) {Governs};
\draw[very thick, dashed] (-5.4,-2.8) -- (-7.4,-1.2);
\draw[very thick, dashed] (-8.6,-2.8) -- (-6.8,-1.2);
\node at (-5.2,-1.8) {Governs};
\draw[very thick, dashed] (-2.2,-2.8) -- (-3.8,-1.2);
\draw[very thick, dashed] (-2.2,-2.8) -- (-3.2,-1.2);
\node at (-1.4,-1.8) {Governs};
\draw[very thick, dashed] (1,-2.8) -- (-0.2,-1.2);

\draw[very thick, dotted] (-13.4,-2.8) ellipse (1.5 and 0.5);
\fill[black!30!green] (-14,-3) ellipse (0.3 and 0.1);
\fill[black!30!green] (-12.8,-2.8) ellipse (0.3 and 0.1);
\fill[black!10!red] (-14,-2.6) ellipse (0.3 and 0.1);
\fill[black!30!green] (-13.2,-2.6) ellipse (0.3 and 0.1);

\draw[very thick, dotted] (-10.2,-2.8) ellipse (1.5 and 0.5);
\fill[black!30!green] (-10.8,-2.8) ellipse (0.3 and 0.1);
\fill[black!30!green] (-9.6,-2.6) ellipse (0.3 and 0.1);

\draw[very thick, dotted] (-7,-2.8) ellipse (1.5 and 0.5);
\fill[black!30!green] (-6.2,-2.8) ellipse (0.3 and 0.1);
\fill[black!10!red] (-7.2,-3) ellipse (0.3 and 0.1);
\fill[black!10!red] (-7.6,-2.6) ellipse (0.3 and 0.1);
\fill[black!30!green] (-6.8,-2.6) ellipse (0.3 and 0.1);

\draw[very thick, dotted] (-3.8,-2.8) ellipse (1.5 and 0.5);
\fill[black!30!green] (-4.4,-3) ellipse (0.3 and 0.1);
\fill[black!30!green] (-4.4,-2.6) ellipse (0.3 and 0.1);
\fill[black!10!red] (-3,-2.6) ellipse (0.3 and 0.1);

\draw[very thick, dotted] (-0.6,-2.8) ellipse (1.5 and 0.5);
\fill[black!30!green] (-1.2,-3) ellipse (0.3 and 0.1);
\fill[black!30!green] (0.4,-2.8) ellipse (0.3 and 0.1);
\fill[black!30!green] (-1.2,-2.6) ellipse (0.3 and 0.1);
\fill[black!30!green] (-0.4,-2.6) ellipse (0.3 and 0.1);
\fill[black!30!green] (-0.4,-3) ellipse (0.3 and 0.1);

\node at (1.2,4.6) {\parbox{20mm}{Highest-level}};
\node at (1.4,1.6) {\parbox{20mm}{Second-level}};
\node at (2.8,-0.6) {\parbox{40mm}{First-level}};
\node at (3.4,-2.8) {\parbox{40mm}{MASs}};
\end{tikzpicture}

==> chapter-6-rulechangeconstitution/Proofs/ProofLemma1.tex <==
\begin{proof} Given the assumptions the proof follows from the definitions:
\begin{enumerate}
\item We have $\forall X \in \pazocal{X} : S^{\prime}_{j:h} \models_{M} X \Leftrightarrow S^{\prime \prime}_{j:h} \models_{M^{\prime \prime}} X$ from \ref{eqNextSucc1}, \ref{eqNextSucc2} and definition~\ref{defModCont}.
\item We will show $E^{\prime \prime}_{j:h} = \textit{GR}(S^{\prime \prime}_{j:h}, O_h, M^{\prime \prime})$:
\begin{enumerate}[label=\roman*]
\item We have $E^{\prime \prime}_{j:h} = \textit{GR}(S^{\prime \prime}_{j:h}, O_h, M^{\prime})$ from \ref{eqSIO2}.
\item $R^{\prime}(i) = R^{\prime \prime}(i)$ from \ref{eqNextSucc3} and \ref{eqSIO4}.
\item From 1, 2.i and 2.ii we have the same conditions for $\textit{GR}(S^{\prime \prime}_{j:h}, O_h, M^{\prime})$ and $\textit{GR}(S^{\prime \prime}_{j:h}, O_h, M^{\prime \prime})$.
\end{enumerate}
From 2.iii and definition~\ref{defGR} we have $E^{\prime \prime}_{j:h} = \textit{GR}(S^{\prime \prime}_{j:h}, O_h, M^{\prime})$.
\item $S^{\prime \prime}_{j:h+1} = \textit{TR}(S^{\prime}_{j:h}, E^{\prime \prime}_{j:h}, M^{\prime \prime})$ - from 1 and definition~\ref{defTR}.
\end{enumerate}
\end{proof}

==> chapter-6-rulechangeconstitution/Proofs/ProofLemma2.tex <==
\begin{proof} A proof can be obtained by structural induction and applying Lemma~\ref{thNextSucc} such that assuming interpretations $\textit{SUCC}_{i}(M, \textit{et})$ and $\textit{SUCC}_{i+1}(M, \textit{et})$ meet the conditions of Lemma~1 there is a third interpretation $\textit{SUCC}_{i+2}(M, \textit{et})$ that is either a fixed point or meets Lemma~\ref{thNextSucc}'s conditions. Potentially by only choosing rule modifications that in $\textit{SUCC}_{i+2}(M, \textit{et})$ that are in $\textit{SUCC}_{i+1}(M, \textit{et})$, and only selecting rule modifications in $\textit{SUCC}_{i+1}(M, \textit{et})$ that are in $\textit{SUCC}_{i+2}(M, \textit{et})$ in the latter case potentially removing rule modifications in all preceding interpretations.
\begin{itemize}
\item[] \textbf{Base case:}
\begin{enumerate}
\item Let $M^{\prime}$ and $M^{\prime \prime}$ be interpretations s.t. 
\begin{enumerate}[label=\roman*]
\item $M^{\prime} = \textit{SUCC}_{0}(\textit{M, et})$ and $M^{\prime \prime} = \textit{SUCC}(M^{\prime}, \textit{et}) = \textit{SUCC}_{1}(\textit{M, et})$ where $\langle S^{\prime}_{0:0} \rangle = \langle S^{\prime \prime}_{0:0} \rangle$ from \ref{eqSIO1}.
\item $\forall i \in [0,k] : \textit{mod(op, id, 0)} \in E^{\prime}_{0:i}, R^{\prime}(i) \leq j \Leftrightarrow \textit{mod(op, id, 0)} \in E^{\prime \prime}_{0:i}, R^{\prime \prime}(i) \leq j$ from \ref{eqGR4}, we can always arbitrarily select rule modification events to \textit{not} occur in both interpretations.
\end{enumerate}
\end{enumerate}
\item[] \textbf{Inductive hypothesis:} Assume that $\forall h \in [0,k], g \in [0,h], j \in [0,v^{\prime \prime}]$ we always have interpretations $M^{\prime} = \textit{SUCC}_{t}(\textit{M, et})$ and $M^{\prime \prime} = \textit{SUCC}_{t+1}(\textit{M, et})$ that share past versions up to the version $j$ and in version $j$ past states up to the time instant $h$ with the same events modifying rules before time instant $h$ at time instants $g$ such that $\forall i \in [0,k]:$
\begin{enumerate}
\item $\langle V^{\prime}_0, ..., V^{\prime}_{j-1} \rangle = \langle V^{\prime \prime}_0, ..., V^{\prime \prime}_{j-1} \rangle$
\item $\langle S^{\prime}_{j:0}, ..., S^{\prime}_{j:h} \rangle = \langle S^{\prime \prime}_{j:0}, ..., S^{\prime \prime}_{j:h} \rangle$
\item $\textit{mod(op, id, g)} \in E^{\prime}_{j:i}, R^{\prime}(i) \leq j \Leftrightarrow \textit{mod(op, id, g)} \in E^{\prime \prime}_{j:i}, R^{\prime \prime}(i) \leq j$.
\end{enumerate}
Either $M^{\prime} = \textit{SUCC}_{t}(\textit{M, et}) = M^{\prime \prime} = \textit{SUCC}_{t+1}(\textit{M, et}) = \textit{SUCC}^{\omega}(\textit{M, et})$ meaning we have found a fixed point. Or, from lemma~\ref{thNextSucc} we have $E^{\prime \prime}_{j:h} = \textit{GR}(S^{\prime}_{j:h}, O_h, M^{\prime})$ and $S^{\prime \prime}_{j:h+1} = \textit{TR}(S^{\prime}_{j:h}, E^{\prime \prime}_{j:h}, M^{\prime})$.
\item[] \textbf{Inductive step:} By the inductive hypothesis let $M^{\prime} = \textit{SUCC}_{t}(\textit{M, et})$ and \\$M^{\prime \prime} = \textit{SUCC}_{t+1}(\textit{M, et})$ be interpretations s.t. $\exists h \in [0,k], j \in [0,v^{\prime \prime}] : \langle V^{\prime}_0, ..., V^{\prime}_{j-1} \rangle = \langle V^{\prime \prime}_0, ..., V^{\prime \prime}_{j-1} \rangle, \langle S^{\prime}_{j:0}, ..., S^{\prime}_{j:h} \rangle = \langle S^{\prime \prime}_{j:0}, ..., S^{\prime \prime}_{j:h} \rangle, \\ \textit{mod(op, id, h)} \in E^{\prime}_{j:i}, R^{\prime}(i) \leq j \Leftrightarrow \textit{mod(op, id, h)} \in E^{\prime \prime}_{j:i}, R^{\prime \prime}(i) \leq j$. One of the following cases holds:
\begin{enumerate}[label=\roman*]
\item[] \textbf{Case 1:} If $h = k$ and $j = v$ then $M^{\prime} = \textit{SUCC}_{t}(\textit{M, et}) = M^{\prime \prime} = \textit{SUCC}_{t+1}(\textit{M, et}) = \textit{SUCC}^{\omega}(\textit{M, et})$ and we have a fixed point.
\item[] \textbf{Case 2:} If $j \neq v$ then we have a third interpretation $M^{\prime \prime \prime} = \textit{SUCC}(M^{\prime \prime}, \textit{et}) = \textit{SUCC}_{t+2}(\textit{M, et})$. We will show that $\forall i \in [0, k] : \langle V^{\prime \prime}_0, ..., V^{\prime \prime}_{j-1} \rangle = \langle V^{\prime \prime \prime}_0, ..., V^{\prime \prime \prime}_{j-1} \rangle\\, \langle S^{\prime \prime}_{j:0}, ..., S^{\prime \prime}_{j:h} \rangle = \langle S^{\prime \prime \prime}_{j:0}, ..., S^{\prime \prime \prime}_{j:h} \rangle, \textit{mod(op, id, h)} \in E^{\prime \prime}_{j:i}, R^{\prime \prime}(i) \leq j \Leftrightarrow \textit{mod(op, id, h)} \in E^{\prime \prime \prime}_{j:i}, R^{\prime \prime \prime}(i) \leq j$:
\begin{enumerate}[label=\roman*]
\item By the inductive hypothesis we can always obtain a fragment of the interpretations $M^{\prime}$ and $M^{\prime \prime}$ which are equivalent up until any time instant $h^{\prime}$ and version $j^{\prime}$ before time instant $h$ in version $j$ with the same events modifying rules before $h^{\prime}$ in the version $j^{\prime}$. Formally: 
\begin{itemize}
\item[] $\forall h^{\prime} \in [0,h], g^{\prime} \in [0,h^{\prime}], j^{\prime} \in [0,j], \forall i \in [0,k] : \langle V^{\prime}_0, ..., V^{\prime}_{j^{\prime}-1} \rangle =\\ \langle V^{\prime \prime}_0, ..., V^{\prime \prime}_{j^{\prime}-1} \rangle, \\ \textit{mod(op, id,} g^{\prime}) \in E^{\prime}_{j^{\prime}:i^{\prime}}, R^{\prime}(i^{\prime}) \leq j^{\prime} \Leftrightarrow \\ \textit{mod(op, id,} g^{\prime}) \in E^{\prime \prime}_{j^{\prime}:i^{\prime}}, R^{\prime \prime}(i^{\prime}) \leq j^{\prime}$ and
\item[] $\forall h^{\prime} \in [0,k], g^{\prime} \in [0,h^{\prime}], j^{\prime} \in [0,j-1], \forall i \in [0,k] : \langle V^{\prime}_0, ..., V^{\prime}_{j^{\prime}-1} \rangle =\\ \langle V^{\prime \prime}_0, ..., V^{\prime \prime}_{j^{\prime}-1} \rangle, \\ \textit{mod(op, id,} g^{\prime}) \in E^{\prime}_{j^{\prime}:i^{\prime}}, R^{\prime}(i^{\prime}) \leq j^{\prime} \Leftrightarrow \\ \textit{mod(op, id,} g^{\prime}) \in E^{\prime \prime}_{j^{\prime}:i^{\prime}}, R^{\prime \prime}(i^{\prime}) \leq j^{\prime}$
\end{itemize}
\item From i and lemma~\ref{thNextSucc} this implies that in the interpretation $M^{\prime \prime}$ all states and event transitions up until time $h$ in version $j$ are produced by $\textit{GR}$ and $\textit{TR}$ passed the interpretation $M^{\prime \prime}$ itself. Formally:
\begin{itemize}
\item[] $\forall h^{\prime} \in [0,h] : E^{\prime \prime}_{j:h^{\prime}} = \textit{GR}(S^{\prime \prime}_{j:h^{\prime}}, O_{h^{\prime}}, M^{\prime \prime}), S^{\prime \prime}_{j:h^{\prime} + 1} = \textit{TR}(S^{\prime \prime}_{j:h^{\prime}}, E^{\prime \prime}_{j:h^{\prime}}, M^{\prime \prime})$ and
\item[] $\forall h^{\prime} \in [0,k], j^{\prime} \in [0, j-1] : E^{\prime \prime}_{j^{\prime}:h^{\prime}} = \textit{GR}(S^{\prime \prime}_{j^{\prime}:h^{\prime}}, O_{h^{\prime}}, M^{\prime \prime}), S^{\prime \prime}_{j^{\prime}: h^{\prime} + 1} = \\ \textit{TR}(S^{\prime \prime}_{j^{\prime}:h^{\prime}}, E^{\prime \prime}_{j^{\prime}:h^{\prime}}, M^{\prime \prime})$.
\end{itemize}
\item From \ref{eqSIO1} every successor interpretation has the same initial states in each version, by this fact, ii, \ref{eqSIO2} and \ref{eqSIO3} and induction we can obtain the interpretation $M^{\prime \prime \prime}$ as being equivalent to $M^{\prime \prime}$ up until time instant $h + 1$ in version $j$, formally: $\langle V^{\prime \prime}_0, ..., V^{\prime \prime}_{j-1} \rangle = \langle V^{\prime \prime \prime}_0, ..., V^{\prime \prime \prime}_{j-1} \rangle, \langle S^{\prime \prime}_{j:0}, ..., S^{\prime \prime}_{j:h+1} \rangle = \langle S^{\prime \prime \prime}_{j:0}, ..., S^{\prime \prime \prime}_{j:h+1} \rangle$
\item We will now show that for each time instant in version $v$ the events that can modify rules before or at the same time as $h+1$ are the same in both $M^{\prime \prime}$ and $M^{\prime \prime \prime}$, formally: $\forall g \in [0, h+1], i \in [0,k]: \textit{mod(op, id, g)} \in E^{\prime \prime}_{j:i}, R^{\prime \prime}(i) \leq j \Leftrightarrow \textit{mod(op, id, g)} \in E^{\prime \prime \prime}_{j:i}, R^{\prime \prime \prime}(i) \leq j$.
\begin{itemize}
\item[] $\forall g \in [h+1], i \in [0,k] : \textit{mod(op, id, g)} \in E^{\prime \prime \prime}_{j:i}, R^{\prime \prime \prime}(i) \leq j \Rightarrow \textit{mod(op, id, g)} \in E^{\prime \prime \prime}_{g:i}, R^{\prime \prime}(i) \leq j$, if $\textit{mod(op, id, g)} \not \in E^{\prime \prime}_{j:i}$ then from \ref{eqGR4} we can arbitrarily select $\textit{mod(op, id, g)} \not \in E^{\prime \prime \prime}_{j:i}$. 
\item[] $\forall g \in [h+1], i \in [0,k]: \textit{mod(op, id, g)} \in E^{\prime \prime \prime}_{j:i}, R^{\prime \prime}(i) \leq j \Rightarrow \textit{mod(op, id, g)} \in E^{\prime \prime \prime}_{j:i}, R^{\prime \prime \prime}(i) \leq j$, if $\textit{mod(op, id, g)} \not \in E^{\prime \prime \prime}_{j:i}$ then from \ref{eqGR4} $\textit{mod(op, id, g)} \not \in E^{\prime \prime}_{j:i}$, note that this choice can be applied in descent for all predecessors.
\end{itemize}
\end{enumerate}
From iii and iv we have shown $\forall i \in [0, k] : \langle V^{\prime \prime}_0, ..., V^{\prime \prime}_{j-1} \rangle = \langle V^{\prime \prime \prime}_0, ..., V^{\prime \prime \prime}_{j-1} \rangle, \\ \langle S^{\prime \prime}_{j:0}, ..., S^{\prime \prime}_{j:h} \rangle = \langle S^{\prime \prime \prime}_{j:0}, ..., S^{\prime \prime \prime}_{j:h} \rangle, \textit{mod(op, id, h)} \in E^{\prime \prime}_{j:i}, R^{\prime \prime}(i) \leq j \Leftrightarrow \textit{mod(op, id, h)} \in E^{\prime \prime \prime}_{j:i}, R^{\prime \prime \prime}(i) \leq j$.
\end{enumerate}
Cases 1 and 2 prove the inductive step.
\end{itemize}
We have shown there exists an $\textit{SUCC}^{\omega}(M, et)$.
\end{proof}

==> conclusion/conclusion.tex <==
\chapter{Conclusion}
\label{conclusion}

This is a concluding chapter explaining the scientific and technical
implications for society of the research findings in considerable detail.


==> epilogue/epilogue.tex <==
\chapter*{Epilogue}
\addcontentsline{toc}{chapter}{Epilogue}
\label{epilogue}

This is an optional epilogue.


==> images/multi_level_example_wb.tex <==
\def\State at (#1,#2,#3,#4){
\coordinate (Pos) at (#1+0.085,#2+0.1);
\draw 		[thick, ->, color=blue] (Pos) arc (180:-55:0.05);
\node [above, color=blue] at (#1+0.15,#2+0.15) {abstraction};

\draw (#1,#2) [black][rounded corners=1pt] ++(0,0) rectangle +(0.16,0.1);
\node [above right] at (#1,#2) {$S_{#4}^{\textit{#3}}$};
}

\def\InstEvo at (#1,#2,#3,#4){

\coordinate (S0) at (#1+-0.185,#2+0.6);
\State at (#1+-0.185,#2+0.6,#3,0)
\draw (S0) [->, very thick] +(0.16,0.05) -- +(0.485,0.05);
\node [above] at (#1+0.15,#2+0.65) {Events$_{0}^{\textit{#3}}$};

\coordinate (S1) at (#1+0.3,#2+0.6);
\State at (#1+0.3,#2+0.6,#3,1)
\draw (S1) [->, very thick] +(0.16,0.05) -- +(0.485,0.05);
\node  [above] at (#1+0.635,#2+0.65) {Events$_{1}^{\textit{#3}}$};

\coordinate (S2) at (#1+0.785,#2+0.6);
\State at (#1+0.785,#2+0.6,#3,2);
\draw (S2) [->, very thick] +(0.16,0.05) -- +(0.485,0.05);
\draw (#1,#2) [fill][white] +(1.05,0.6) rectangle +(1.15,0.7);
\node [above, font=\bf] at (#1+1.1,#2+0.6) {$...$};

\State at (#1+1.27,#2+0.6,#3,k+1);

\node [above right,font=\bf] at (#1+-0.25, #2+0.85) {#4};
\draw (#1,#2)[black][thick,rounded corners=3pt] +(-0.25,0.575) rectangle +(1.6,0.85);
}

\def\ObsEvent at (#1,#2,#3,#4){
\coordinate (Pos) at (#1+0.085,#2+0.1);
\draw 		[thick, ->] (Pos) arc (180:-55:0.05);
\node [above] at (#1+0.15,#2+0.15) {abstraction};

\draw (#1,#2) [black][rounded corners=1pt] ++(0,0) rectangle +(0.16,0.1);
\node [above right] at (#1,#2) {$S_{#4}^{\textit{#3}}$};
}

\def\ObsTrace at (#1,#2){

\coordinate (S0) at (#1+-0.185,#2+0.6);

\node [above] at (#1+0.15,#2+0.65) (ObEv0) {Obs. Event$_{0}$};
\node  [above] at (#1+0.635,#2+0.65) (ObEv1) {Obs. Event$_{1}$};
\node  [above] at (#1+1.12,#2+0.65) (ObEvk) {Obs. Event$_{k}$};
\draw [->, very thick] (ObEv0.east) -- (ObEv1.west);
\draw [->, very thick] (ObEv1.east) -- (ObEvk.west);

\draw (#1,#2) [fill][white] +(0.8,0.6) rectangle +(0.9,0.7);
\node [above, font=\bf] at (#1+0.85,#2+0.6) {$...$};

}
\begin{tikzpicture}[xscale=5.5,yscale=5.5]
\InstEvo at (0,1,n,Nth-level Institution)
\InstEvo at (0,0.5,2,Second-level Institution)
\InstEvo at (0,0,1,First-level Institution)

\ObsTrace at (0,-0.4)

\fill (0.675,1.522) circle (0.13mm);
\fill (0.675,1.472) circle (0.13mm);
\fill (0.675,1.422) circle (0.13mm);

\draw [line width=1.5mm,
preaction={-triangle 90,line width=0.8mm,draw,shorten >=-1mm}] (0.675,0.880) -- (0.675,1.005);
\node [above right, text width = 3cm] at (0.75, 0.9) {Link};

\draw [line width=1.5mm,
preaction={-triangle 90,line width=0.8mm,draw,shorten >=-1mm}] (0.675,0.375) -- (0.675,0.5);
\node [above right, text width = 3cm] at (0.75, 0.4) {Input for all Institutions};

\end{tikzpicture}


==> preface/preface.tex <==
\chapter*{Preface}
\addcontentsline{toc}{chapter}{Preface}
\setheader{Preface}

Preface goes here. This chapter is optional.

\begin{flushright}
{\makeatletter\itshape
    \@firstname\ \@lastname \\
    Delft, January 2013
\makeatother}
\end{flushright}



==> publications/publications.tex <==
\chapter*{List of Publications}
\addcontentsline{toc}{chapter}{List of Publications}
\setheader{List of Publications}
\label{publications}

%% We use the 'etaremune' environment (the reverse of 'enumerate') to get a
%% numbered list of publications in reverse chronological order. If the list of
%% authors is long, it might be useful to emphasize your own name with \textbf.
\begin{etaremune}{\small

\item \textbf{A.\ Einstein}, \textit{Ist die Tr\"agheit eines K\"orpers von seinem Energieinhalt abh\"angig?}, \href{http://dx.doi.org/10.1002/andp.19053231314}{Annalen der Physik \textbf{18}, 639 (1906)}.
\item \textbf{A.\ Einstein}, \textit{Zur Elektrodynamik bewegter K\"orper}, \href{http://dx.doi.org/10.1002/andp.19053221004}{Annalen der Physik \textbf{17}, 891 (1905)}.
\item \textbf{A.\ Einstein}, \textit{\"Uber die von der molekularkinetischen Theorie der W\"arme geforderte Bewegung von in ruhenden Fl\"ussigkeiten suspendierten Teilchen}, \href{http://dx.doi.org/10.1002/andp.19053220806}{Annalen der Physik \textbf{17}, 549 (1905)}.
\item \textbf{A.\ Einstein}, \textit{\"Uber einen die Erzeugung und Verwandlung des Lichtes betreffenden heuristischen Gesichtspunkt}, \href{http://dx.doi.org/10.1002/andp.19053220806}{Annalen der Physik \textbf{17}, 132 (1905)}.

}\end{etaremune}



==> summary/summary_before_removing.tex <==
\chapter*{Summary}
\addcontentsline{toc}{chapter}{Summary}
\setheader{Summary}

%\textbf{Short description:} Institution designers (e.g. governments) design institutions (e.g. legislation) comprising rules and regulations to guide societies towards `legal' behaviour. But how can we determine if institution designers are acting legally? Institution designers can design institutions which are illegal, such as by placing unacceptable limits on people's rights. Moreover, the design process can be illegal, such as by changing rules without following the processes which regulate rule change. This thesis contributes practical formal reasoning for automatically assessing whether institution designs are legal and whether they are are designed and changed in a legal way.

\begin{comment}
\textbf{Short description:} Governments design institutions comprising rules and regulations. Governments are also governed. This is with rules and regulations, which guide them towards designing `correct' institutions (e.g. those that do not place unacceptable limits on people's rights) in a `correct' way (e.g. following procedures stating how an institution can be changed, when and by whom). This thesis aims to support institution designers, with automated reasoning, in designing correct institutions in a correct way and external monitors in assessing institution designers are behaving correctly. This thesis contributes formal reasoning for automatically assessing when institution designers, such as governments, are abiding by the regulations placed on them.
\end{comment}

The work presented in this thesis is motivated by the need for a precise way to evaluate the consequences of the constraints placed on governments, organisations, contract writers and other regulatory bodies. If an organisation wishes to meet various aims by engaging in contracts for resources to participate in the organisation, such as collecting data by contracting people's time and effort in answering queries. Then, the organisation's contracts \textit{should} abide by external laws such as by maintaining human rights. Furthermore, the contracts \textit{can} only be enacted if the organisation follows contract law processes, such as by ensuring there is bilateral agreement and consideration. If a  national government wishes to legislate appropriately to guide a society and serve its own interests, then it must be aware of the national and international governance hierarchy context it operates in. Modern governments \textit{should} respect constraints from directives, international treaties and human rights charters, which guide the legislation governments enact, or face punishment. Moreover, governments \textit{can} only enact legislation by following law making rules, such as a majority vote and constraints on the scope and types of law being enacted. In general, these are all examples of institutions, such as laws and contracts, being designed and enacted under constraints. The common thread binding these examples is that institution designers are loosely tied in how the institutions they enact \textit{should} be designed and strongly tied in how and when they \textit{can} enact institutional changes.

However, such constraints placed on institution designers appear intangible, making it hard to grasp exactly how to operate within them. Without precise notions for how an institution \textit{should} be designed with respect to external laws, how can an institutional designer, such as a national government, predict whether a judiciary would find them guilty of enacting a `bad' design in order to avoid punishment? As citizens governed in a society, how can we have a common understanding of which laws are in place and when? In particular, based on the actions governments take with respect to the constraints defining how and when they can enact institutional changes. Moreover, it becomes hard to say whether such constraints are being reasoned about `correctly' when vague sentiments are put in place of precise operational details. How would we know if there are fundamental flaws in the constraints' typical operationalisation, causing punishments where there should be none, if the operationalisation is not somehow laid bare in front of us? Finally, if it is fundamentally arduous to make decisions under such constraints, such as what to do in order to enact a law, given their ambiguity how can we offer computerised decision support? In other words, what we need to do is take such informal concepts and give them \textit{form} in order to make it clear how to assess constraints placed on institutional designs and enacting changes, automate decision making over how best to behave within those constraints, and analyse whether the underlying reasoning is acceptable or not.

The goal of this thesis is to give a rigorous mathematical account of constraints placed on institutional designs and enacting institutional changes, taking a formalist's perspective to social constructions. Moreover, 

% Moreover, as citizens governed in a society, how can we be sure what blahs we operate on given that they are blahed? Moreover, how can we be sure the way in which blah is reasoned about is `correct' if that reasoning has no form for us to critique? What if all this blah is too complicated for humans to deal with, given that they are all vague and so on blah blah how can we alleviate our burden on checking such and such through automation without a clear ideaa of what these concepts are to the extent a computer can `understand' them? What if we want to rectify such mistakes as so on through automation? In other words, how can we take these informal concepts of ... and give them form? That is the goal of this thesis, which contributes a mathematically rigorous formal reasoning for governing institution design and change to support communicating the concepts clearly, analysing those concepts and automating the reasoning etc. etc. (make this short)

% Institutions, in this sense, are sets of rules and regulations make possible social actions... guide agent behavior... (then talk about this thesis) Whilst much work has focussed on the former, this thesis looks at... from the perspective that... it defines concepts, automates, etc. etc.
% explain institutions here and move to what is being formalised

% Formalisation is a conceptualisation approach to...
% In the same way a judiciary would...



More generally, this thesis aims to support a wide range of cases where people are governed or occasionally adopt a legislative role, from people \textit{agreeing} to contribute data collected from their cellphone sensors, to stakeholders in sensor networks in \textit{designing} `correct' institutions to govern those networks, to legislators in the traditional sense of national governments.

Governments govern societies towards `good' outcomes as envisioned by the ruling body. This is by designing institutions, which impose rules and regulations on society's members, with rewards for good behaviour and punishments for bad behaviour. However, governments are capable of designing new institutions or changing existing institutions in an incorrect way. For example, governments might be designing institutions that lack coordination with institutions governing other jurisdictions (e.g. environmental regulations lacking coordination between nation states for cohesive cross-national environmental governance) or that place unacceptable limits on agents rights (e.g. rights to privacy). Moreover, governments might not be following an institution design process. Institution design processes being the set of rules and regulations that govern the process of legislating, stating how and when an institution can be changed and by whom. Consequently, modern governance does not exist in isolation free from control. 

Rather, governments are also governed by institutions. These institutions regulate how and when governments \textit{can} change their own institutions and what institution designs they \textit{should} impose on agents. Just as agents acting in a society can be punished for not following institution regulations, so too are governments punished for not following institutional regulations governing the way in which they change and design institutions. This is problematic, since a government is burdened with manually checking it is designing correct institutions in a correct way, and similarly for third-parties whose role it is to enforce correct governance and punish bad governance (e.g. courts or other governments). A possible solution is to automate reasoning about institutional regulations which govern the way in which institutions can be changed and designed. On the one hand, artificial intelligence has contributed automated institutional reasoning, with deontic logics and other formalisms, for societal members to determine how to comply with institutions, and governments in which members of a society should be rewarded and punished and when. On the other hand, little attention has been paid to reasoning about the governance of government. This thesis addresses this issue by contributing the PARAGON framework, comprising \textbf{P}ractical \textbf{A}utomated \textbf{R}easoning for \textbf{A}ssessing \textbf{Go}ver\textbf{n}ance in how institutions are designed and the actual designs enacted.

The framework has a wide application area and was conducted under the SHINE project\footnote{\url{http://shine.tudelft.nl}} (Sensing Heterogeneous Information Network Environment) which, in part, involves governing large-scale heterogeneous sensor networks. In the SHINE project an objective was to gather novel environmental data by using existing, potentially unused, environmental sensors and sensor networks contributed by different stakeholders. For example, one sensor network could be rain radars contributed by a municipality, whilst another network could gather crowdsourced localised audio data with the cellphones of ordinary people running a cellphone application. Different sensor networks contribute heterogeneous data types which can collectively be used to come to new conclusions, such as existing and future crowding levels using cellphone audio and weather radar data. This thesis contributes reasoning for governing such sensor networks, which due to comprising autonomous agents (e.g. municipalities, people running cellphone apps) might not be controllable directly. Firstly, with reasoning for sensor networks being governed by institutions whose rules can be changed over time as different governance needs for the sensor network arise (e.g. as the data needs change or as it emerges previous rules were inadequate). Secondly, by contributing reasoning for designing institutions which individually govern separate sensor networks (e.g. software policies regulating people in keeping a cellphone speaker on) which in turn require coordinated regulations with each other to meet a more global goal (i.e. gathering data) without placing unacceptable limits on people's rights (e.g. violating the right to privacy). The same reasoning also supports people considering whether to contribute their sensors (e.g. on their cellphone) without losing certain rights they value highly. Thirdly, by supporting the stakeholders of the sensor networks with automated institution re-design recommendations to ensure the institutions are designed `correctly'.

This thesis meets these aims in three ways. Firstly, by contributing a formalisation of rule change governed by rules, with the aim of contributing a flexible rule change system. The starting point is to view institutions as containing definitional rules giving meaning to various institutional concepts. Known as Searle's constitutive rules, these are rules of the form ``A counts-as B in context C'', which build a social reality from brute facts and regulate social reality change when the brute facts change. For example, ``a piece of paper with certain European Union symbols counts-as money in the context of the European Union''. This thesis looks at counts-as rule changes which are also regulated by \textit{rule-modifying} counts-as rules ascribing rule change in the past/present/future (e.g. a government voting to change a rule \textit{counts-as} a rule change). Determining rule change legality is difficult, since changing counts-as rules alters the social reality which rule changes are conditional on. Moreover, because rule changes can be conditional on the effect they \textit{would} have (e.g. not criminalising formerly innocent people). This thesis answers ``when do rule changes count-as legal rule changes?'' with a novel formal framework for rule change ascribed by past/present/future rule modifying counts-as rules.

Secondly, by contributing reasoning for governments whose institution designs are governed towards being coordinated with other institutions and not placing unacceptable limits on agents' rights. Here the reasoning deals with what is called \textit{multi-level governance}, where institution designs at lower-levels of governance (e.g. national legislation at the national level) are governed by higher-level institutions (e.g. directives, human rights charters and supranational agreements). When an institution design is found to be non-compliant, punishments can be issued by annulling the legislation or imposing fines on the responsible designers (i.e. government). To enforce multi-level governance, higher-levels of government must check lower-levels for compliance; in order to avoid punishment lower-levels must check their institution designs are compliant before enactment. Yet, checking non-compliance of institution designs in multi-level governance is non-trivial. In particular, because institutions in multi-level governance operate at different levels of abstraction. Lower-level institutions govern with concrete regulations whilst higher-level institutions comprise increasingly vague and abstract regulations. For example, national legislation concretely obliges communications providers to store citizen's communications data, whilst a human rights charter abstractly prohibits unfair data processing. Somehow, it must be assessed whether concretely obliging storing citizen's communications data violates abstract regulations on unfair data processing. Somehow, concrete regulations must be checked for compliance with abstract regulations. This thesis contributes automated compliance checking for multi-level governance, both from a formal theoretical point of view and from a practical standpoint with a corresponding computational framework.

Thirdly, this thesis contributes a computational mechanism for changing non-compliant institution designs in multi-level governance, coming back to the idea of institution rule change. For a designer of a non-compliant institution there remains a dilemma: be punished for non-compliant regulations or arduously determine and rectify the underlying causes of non-compliance. This thesis contributes a way to automatically determine how to revise an institution to be compliant. In particular, whilst the trivial case of removing all institution rules is often possible, effectively not enacting the institution. Specifically, this thesis addresses the need to minimise the change in an institutions regulations' outcomes. Potentially, changing rules in a fine grained way or adding entirely new rules. The objective is to ensure after an institution is revised to be compliant, the various obligations, prohibitions and other normative effects it imposes are as close as possible to when the institution was non-compliant. Thus, keeping as closely as possible to the institution designers' original intentions.

Furthermore, this thesis aims to make both philosophical and practical contributions. From the philosophical side, this thesis aims to formalise previously informal notions provided by political science and legal philosophy. Specifically, to provide precise conceptualisations for rules which govern rule change and institutions which govern institution designs. Particular attention is paid to understanding the new conceptualisations and assessing them against a number of case studies. The case studies are used to assess whether the formal contributions provide `correct' outcomes (i.e. inferences). From the practical side, the contributed reasoning is either coupled with an implementation or a computational characterisation of the formal concepts providing necessary details for implementation. To summarise, this thesis aims to contribute new philosophical conceptualisations and practical ways to implement them in the area of governance of government; this thesis lies at the intersection of \textit{legal philosophy and symbolic artificial intelligence}.

%\chapter*{Samenvatting}
%\addcontentsline{toc}{chapter}{Samenvatting}
%\setheader{Samenvatting}

%{\selectlanguage{dutch}

%Samenvatting in het Nederlands\ldots

%}



==> summary/summary_before_removing_2.tex <==
\chapter*{Summary}
\addcontentsline{toc}{chapter}{Summary}
\setheader{Summary}

%\textbf{Short description:} Institution designers (e.g. governments) design institutions (e.g. legislation) comprising rules and regulations to guide societies towards `legal' behaviour. But how can we determine if institution designers are acting legally? Institution designers can design institutions which are illegal, such as by placing unacceptable limits on people's rights. Moreover, the design process can be illegal, such as by changing rules without following the processes which regulate rule change. This thesis contributes practical formal reasoning for automatically assessing whether institution designs are legal and whether they are are designed and changed in a legal way.

\begin{comment}
\textbf{Short description:} Governments design institutions comprising rules and regulations. Governments are also governed. This is with rules and regulations, which guide them towards designing `correct' institutions (e.g. those that do not place unacceptable limits on people's rights) in a `correct' way (e.g. following procedures stating how an institution can be changed, when and by whom). This thesis aims to support institution designers, with automated reasoning, in designing correct institutions in a correct way and external monitors in assessing institution designers are behaving correctly. This thesis contributes formal reasoning for automatically assessing when institution designers, such as governments, are abiding by the regulations placed on them.
\end{comment}

This thesis is motivated by the need, in today's globalist world, for a precise way to enable governments, organisations and other regulatory bodies to evaluate the constraints they place on themselves and one another in order to coordinate and operate successfully. An organisation's modus operandi is enacting and fulfilling contracts between itself and its participants, such as for people's time and effort in answering data-driven queries. Yet, such organisational contracts \textit{should} respect external laws, such as those setting out data privacy rights and liberties. Moreover, those contracts \textit{can} only be enacted by following contract law processes, which require bilateral agreement and consideration. Governments, too, need to legislate whilst understanding today's context of national and international governance hierarchy where law makers shun isolationism and seek to influence one another. Governments \textit{should} avoid punishment by respecting constraints from  international treaties and human rights charters. Moreover, governments \textit{can} only enact legislation by following their own, pre-existing, law making procedures. In general, these are all examples of institutions, such as laws and contracts, being designed and enacted under constraints. The common thread binding these examples is that institution designers, such as organisations and governments, are loosely tied in how the institutions they enact \textit{should} be designed and strongly tied in how and when they \textit{can} enact institutional changes. However, the existence of such constraints makes them no less intangible. We can clearly see they exist even though we cannot physically see them. This makes it hard to grasp exactly how institution designers need to operate under institutional design and enactment constraints.

This thesis contributes the PARAGon framework, which makes constraints placed on institution designers clear and precise. \textit{Formalisation} is the main technique used, which provides a mathematically rigorous account of, previously informal, constraints placed on institutional designs and enacting institutional changes. Hence, the unseen constraints become seeable, not as physical bindings, but as symbols on a page defining the inferences institution designers need to make in order to understand how they should design institutions and how they can enact those institutions. From a conceptualisation standpoint, the main benefit is that by formalising the operationalisation of such constraints we are firstly able to understand the concepts involved and secondly able to identify fundamental flaws in the formal concepts offered. Or, in the words of Leibniz, ``The only way to rectify our reasonings is to make them as tangible as those of the Mathematicians, so that we can find our error at a glance''. From a practical standpoint there are benefits in two senses. Firstly, by being defined in such a way as to enable automation, which allows delegating to a computer the cognitively difficulty tasks for institution designers to operate inside the constraints and judiciaries to apply the negative consequences of operating outside the constraints. Secondly, by dealing with the pragmatics. The framework is developed with and applied to case studies situated in the law and organisational sensor networks in order to capture the meaning of institutional constraints as they are used in real-world contexts. In other words, this thesis contributes the PARAGon framework for \textbf{P}ractical \textbf{A}utomated \textbf{R}easoning for \textbf{A}ssessing \textbf{Go}ver\textbf{n}ance of institution design and change.

Moreover, the framework's application has practical consequences. Firstly, because the framework can be disseminated in a precise mathematical way to citizens, institution designers and judiciaries alike. This means an institution designer, such as a national government, can avoid punishment by predicting whether a judiciary would find them guilty of enacting a `bad' institution design by applying the same reasoning the judiciary would. Moreover, a judiciary can ensure fairness by applying the same reasoning from case to case. Through automation, an institution designer can apply the framework to search for resolutions

 Citizens of a governed society can have a common understanding of which laws are enacted and when, by applying the framework to the constraints stating what actions an institution designer must stake to enact institutional changes.

, by applying the same formal reasoning a judiciary would enacting a `bad' design in order to avoid punishment? As citizens governed in a society, how can we  have a common understanding of which laws are in place and when? In particular, based on the actions governments take with respect to the constraints defining how and when they can enact institutional changes. Moreover, it becomes hard to say whether such constraints are being reasoned about `correctly' when vague sentiments are put in place of precise operational details. 
  
   Finally, if it is fundamentally arduous to make decisions under such constraints, such as what to do in order to enact a law, given their ambiguity how can we offer computerised decision support? In other words, what we need to do is take such informal concepts and give them \textit{form} in order to make it clear how to assess constraints placed on institutional designs and enacting changes, automate decision making over how best to behave within those constraints, and analyse whether the underlying reasoning is acceptable or not.

 
 
PARAGon framework presented in this thesis rectifies such vagueness by 



The goal of this thesis is therefore, to give a rigorous mathematical account of constraints placed on institutional designs and enacting institutional changes. Moreover, this thesis addresses the practical side. First, from the perspective of contributing formalisation which leads to automation. 

This thesis achieves this goal by contributing the PARAGon framework which formalises \textbf{P}ractical \textbf{A}utomated \textbf{R}easoning for \textbf{A}ssessing \textbf{Go}ver\textbf{n}ance of institutional design and enacting institutional changes. The framework has a wide application area and was conducted under the SHINE project\footnote{\url{http://shine.tudelft.nl}} (Sensing Heterogeneous Information Network Environment) which, in part, involves governing large-scale heterogeneous sensor networks. In the SHINE project an objective was to gather novel environmental data by using existing, potentially unused, environmental sensors and sensor networks contributed by different stakeholders. For example, one sensor network could be rain radars contributed by a municipality, whilst another network could gather crowdsourced localised audio data with the cellphones of ordinary people running a cellphone application. Different sensor networks contribute heterogeneous data types which can collectively be used to come to new conclusions, such as existing and future crowding levels using cellphone audio and weather radar data. This thesis contributes reasoning for governing such sensor networks, which due to comprising autonomous agents (e.g. municipalities, people running cellphone apps) might not be controllable directly. Firstly, with reasoning for sensor networks being governed by institutions whose rules can be changed over time as different governance needs for the sensor network arise (e.g. as the data needs change or as it emerges previous rules were inadequate). Secondly, by contributing reasoning for designing institutions which individually govern separate sensor networks (e.g. software policies regulating people in keeping a cellphone speaker on) which in turn require coordinated regulations with each other to meet a more global goal (i.e. gathering data) without placing unacceptable limits on people's rights (e.g. violating the right to privacy). The same reasoning also supports people considering whether to contribute their sensors (e.g. on their cellphone) without losing certain rights they value highly. Thirdly, by supporting the stakeholders of the sensor networks with automated institution re-design recommendations to ensure the institutions are designed `correctly'.

This thesis meets these aims in three ways. Firstly, by contributing a formalisation of rule change governed by rules, with the aim of contributing a flexible rule change system. The starting point is to view institutions as containing definitional rules giving meaning to various institutional concepts. Known as Searle's constitutive rules, these are rules of the form ``A counts-as B in context C'', which build a social reality from brute facts and regulate social reality change when the brute facts change. For example, ``a piece of paper with certain European Union symbols counts-as money in the context of the European Union''. This thesis looks at counts-as rule changes which are also regulated by \textit{rule-modifying} counts-as rules ascribing rule change in the past/present/future (e.g. a government voting to change a rule \textit{counts-as} a rule change). Determining rule change legality is difficult, since changing counts-as rules alters the social reality which rule changes are conditional on. Moreover, because rule changes can be conditional on the effect they \textit{would} have (e.g. not criminalising formerly innocent people). This thesis answers ``when do rule changes count-as legal rule changes?'' with a novel formal framework for rule change ascribed by past/present/future rule modifying counts-as rules.

Secondly, by contributing reasoning for governments whose institution designs are governed towards being coordinated with other institutions and not placing unacceptable limits on agents' rights. Here the reasoning deals with what is called \textit{multi-level governance}, where institution designs at lower-levels of governance (e.g. national legislation at the national level) are governed by higher-level institutions (e.g. directives, human rights charters and supranational agreements). When an institution design is found to be non-compliant, punishments can be issued by annulling the legislation or imposing fines on the responsible designers (i.e. government). To enforce multi-level governance, higher-levels of government must check lower-levels for compliance; in order to avoid punishment lower-levels must check their institution designs are compliant before enactment. Yet, checking non-compliance of institution designs in multi-level governance is non-trivial. In particular, because institutions in multi-level governance operate at different levels of abstraction. Lower-level institutions govern with concrete regulations whilst higher-level institutions comprise increasingly vague and abstract regulations. For example, national legislation concretely obliges communications providers to store citizen's communications data, whilst a human rights charter abstractly prohibits unfair data processing. Somehow, it must be assessed whether concretely obliging storing citizen's communications data violates abstract regulations on unfair data processing. Somehow, concrete regulations must be checked for compliance with abstract regulations. This thesis contributes automated compliance checking for multi-level governance, both from a formal theoretical point of view and from a practical standpoint with a corresponding computational framework.

Thirdly, this thesis contributes a computational mechanism for changing non-compliant institution designs in multi-level governance, coming back to the idea of institution rule change. For a designer of a non-compliant institution there remains a dilemma: be punished for non-compliant regulations or arduously determine and rectify the underlying causes of non-compliance. This thesis contributes a way to automatically determine how to revise an institution to be compliant. In particular, whilst the trivial case of removing all institution rules is often possible, effectively not enacting the institution. Specifically, this thesis addresses the need to minimise the change in an institutions regulations' outcomes. Potentially, changing rules in a fine grained way or adding entirely new rules. The objective is to ensure after an institution is revised to be compliant, the various obligations, prohibitions and other normative effects it imposes are as close as possible to when the institution was non-compliant. Thus, keeping as closely as possible to the institution designers' original intentions.

Furthermore, this thesis aims to make both philosophical and practical contributions. From the philosophical side, this thesis aims to formalise previously informal notions provided by political science and legal philosophy. Specifically, to provide precise conceptualisations for rules which govern rule change and institutions which govern institution designs. Particular attention is paid to understanding the new conceptualisations and assessing them against a number of case studies. The case studies are used to assess whether the formal contributions provide `correct' outcomes (i.e. inferences). From the practical side, the contributed reasoning is either coupled with an implementation or a computational characterisation of the formal concepts providing necessary details for implementation. To summarise, this thesis aims to contribute new philosophical conceptualisations and practical ways to implement them in the area of governance of government; this thesis lies at the intersection of \textit{legal philosophy and symbolic artificial intelligence}.

%\chapter*{Samenvatting}
%\addcontentsline{toc}{chapter}{Samenvatting}
%\setheader{Samenvatting}

%{\selectlanguage{dutch}

%Samenvatting in het Nederlands\ldots

%}



==> summary/summary_before_removing_3.tex <==
\chapter*{Summary}
\addcontentsline{toc}{chapter}{Summary}
\setheader{Summary}

%\textbf{Short description:} Institution designers (e.g. governments) design institutions (e.g. legislation) comprising rules and regulations to guide societies towards `legal' behaviour. But how can we determine if institution designers are acting legally? Institution designers can design institutions which are illegal, such as by placing unacceptable limits on people's rights. Moreover, the design process can be illegal, such as by changing rules without following the processes which regulate rule change. This thesis contributes practical formal reasoning for automatically assessing whether institution designs are legal and whether they are are designed and changed in a legal way.

\begin{comment}
\textbf{Short description:} Governments design institutions comprising rules and regulations. Governments are also governed. This is with rules and regulations, which guide them towards designing `correct' institutions (e.g. those that do not place unacceptable limits on people's rights) in a `correct' way (e.g. following procedures stating how an institution can be changed, when and by whom). This thesis aims to support institution designers, with automated reasoning, in designing correct institutions in a correct way and external monitors in assessing institution designers are behaving correctly. This thesis contributes formal reasoning for automatically assessing when institution designers, such as governments, are abiding by the regulations placed on them.
\end{comment}

This thesis is motivated by the need, in today's globalist world, for a precise way to enable governments, organisations and other regulatory bodies to evaluate the constraints they place on themselves and one another in order to coordinate and operate successfully. An organisation's modus operandi is enacting and fulfilling contracts between itself and its participants, such as for people's time and effort in answering data-driven queries. Yet, such organisational contracts \textit{should} respect external laws, such as those setting out data privacy rights and liberties. Moreover, those contracts \textit{can} only be enacted by following contract law processes, which require bilateral agreement and consideration. Governments, too, need to legislate whilst understanding today's context of national and international governance hierarchy where law makers shun isolationism and seek to influence one another. Governments \textit{should} avoid punishment by respecting constraints from  international treaties and human rights charters. Moreover, governments \textit{can} only enact legislation by following their own, pre-existing, law making procedures. In general, these are all examples of institutions, such as laws and contracts, being designed and enacted under constraints. The common thread binding these examples is that institution designers, such as organisations and governments, are loosely tied in how the institutions they enact \textit{should} be designed and strongly tied in how and when they \textit{can} enact institutional changes. However, the existence of such constraints makes them no less intangible. We can clearly see they exist even though we cannot physically see them. This makes it hard to grasp exactly how institution designers need to operate under institutional design and enactment constraints.

This thesis contributes the PARAGon framework, which makes constraints placed on institution designers clear and precise. \textit{Formalisation} is the main technique used, which provides a mathematically rigorous account of, previously informal, constraints placed on institutional designs and enacting institutional changes. Hence, the unseen constraints become seeable, not as physical bindings, but as symbols on a page defining the inferences institution designers need to make in order to understand how they should design institutions and how they can enact those institutions. From a conceptualisation standpoint, the main benefit is that by formalising the operationalisation of such constraints we are firstly able to understand the concepts involved and secondly able to identify fundamental flaws in the formal concepts offered. Or, in the words of Leibniz, ``The only way to rectify our reasonings is to make them as tangible as those of the Mathematicians, so that we can find our error at a glance''. From a practical standpoint there are benefits in three senses. Firstly, the formal reasoning is disseminated in clear mathematical reasoning. So, an institution designer applies the exact same reasoning a judiciary would in order to operate within constraints of international law, a judiciary systematically applies the same reasoning fairly from one case to another, and governed citizens have common knowledge of which laws are in place and when by coming to the same understanding of when institution designers enact regulatory changes. Secondly by being defined in such a way as to enable automation, which allows delegating to a computer the cognitively difficulty tasks for institution designers to operate inside the constraints and judiciaries to apply the negative consequences of operating outside the constraints. Thirdly, by dealing with the pragmatics. The framework is developed with and applied to case studies situated in the law and organisational sensor networks in order to capture the meaning of institutional constraints as they are used in real-world contexts. In other words, this thesis contributes the PARAGon framework for \textbf{P}ractical \textbf{A}utomated \textbf{R}easoning for \textbf{A}ssessing \textbf{Go}ver\textbf{n}ance of institution design and change.

The PARAGon framework adopts the well known notion of an institution conceived by Searle as a set of constitutive counts-as rules of the form ``A counts-as B in context C'' and contributes new conceptualisations based on these rules. These rules build a social reality from brute facts and regulate social reality change when the brute facts change. For example, ``a piece of paper with certain European Union symbols counts-as money in the context of the European Union''. The PARAGon framework makes three contributions, using counts-as rules, for formalised and automated reasoning about constraints governing institution design and enactment.

Firstly, PARAGon comprises formalised reasoning for institution designers, such as governments and organisations, whose institution designs are governed towards being coordinated with other institutions and not placing unacceptable limits on agents' rights. Here the reasoning deals with what is called \textit{multi-level governance}, where institution designs at lower-levels of governance (e.g. national legislation at the national level) are governed by higher-level institutions (e.g. directives, human rights charters and supranational agreements). When an institution design is found to be non-compliant, punishments can be issued by annulling the legislation or imposing fines on the responsible designers (i.e. government). Key to multi-level governance is the notion of abstraction. Institutions at higher-levels comprise abstract regulations governing the concrete regulatory effects of lower-levels. This thesis adopts counts-as rules as defining concepts, prescriptions and links between concrete and abstract concepts. The PARAGon framework uses counts-as rules to establish whether concrete regulations in lower governance level institutions can be applied in social contexts such that they violate abstract regulations as set out in directives, human rights charters, and so on.

Secondly, PARAGon contributes a computational mechanism for changing non-compliant institution designs in multi-level governance. For a designer of a non-compliant institution there remains a dilemma: be punished for non-compliant regulations or arduously determine and rectify the underlying causes of non-compliance. This thesis contributes a way to automatically determine how to revise an institution to be compliant. In this case, the framework looks at explanations for non-compliance in the form of changes to counts-as rules which would ensure compliance in different social contexts. In particular, whilst the trivial case of removing all institution rules is often possible, effectively not enacting the institution. Specifically, this thesis addresses the need to minimise the change in an institutions regulations' outcomes. Potentially, changing counts-as rules in a fine grained way or synthesising new counts-as rules. The PARAGon framework offers a compliance explanation and resolution mechanism which keeps as closely as possible to an institution designers' original intentions.

Thirdly, PARAGon formalises constraints placed on when institutions and institutional changes can be enacted. These constraints are legal rules which define how and when other legal rules can be changed. They are also known as secondary rules when compared to the primary rules of a legal system which define concepts and regulate behaviour. PARAGon formalises such secondary rules as \textit{rule-modifying} counts-as rules, which ascribe rule change at various points in time. For example, a government voting to change a rule \textit{counts-as} a rule change. Determining rule change legality is difficult, since changing counts-as rules alters the social reality which rule changes are conditional on. Moreover, because rule changes can be conditional on the effect they \textit{would} have (e.g. not criminalising formerly innocent people). The PARAGon framework contributes formal reasoning for determining when rule changes count-as legal rule changes, according to ascriptions by past/present/future rule modifying counts-as rules.

The PARAGon framework is applied to the law and the SHINE project\footnote{\url{http://shine.tudelft.nl}} (Sensing Heterogeneous Information Network Environment) under which the research was conducted. SHINE, in part, aims to form large-scale heterogeneous sensor networks, using existing sensors in the environment belonging to external stakeholders, to gather detailed environmental data that varies in type. PARAGon aims to support automated governance for large scale heterogeneous `SHINE' sensor networks. Firstly, PARAGon is applicable to supporting the formation of SHINE sensor super-systems of sub-systems, comprising a thin SHINE institution layer abstractly governing the design of sub-system institutions towards coordinated regulations for collecting environmental data collection. The incentive for sub-system stakeholders is that correctly governed sub-systems join a SHINE super-system for sharing data of different types and the benefit for SHINE is that sub-system governance is delegated. Secondly, PARAGon supports sensor network stakeholders with automated institution re-design recommendations to ensure the institutions are designed `correctly'. Thirdly, PARAGon supports automated reasoning for how and when sensor system regulations are changed over time as different governance needs arise (e.g. as the data needs change or as it emerges previous rules were inadequate).

The PARAGon framework makes both formal and practical contributions. From the formal side, this thesis aims to formalise previously informal notions provided by political science and legal philosophy. Specifically, to provide precise conceptualisations for institutions which govern institution designs and rules which govern rule change. Particular attention is paid to understanding the new conceptualisations and assessing them against a number of case studies. The case studies are used to assess whether the formal contributions provide `correct' outcomes (i.e. inferences). From the practical side, the contributed reasoning is either coupled with an implementation or a computational characterisation of the formal concepts providing necessary details for implementation. To summarise, this thesis aims to contribute new formal conceptualisations and practical ways to implement them in the area of governing governance; this thesis lies at the intersection of \textit{legal philosophy and symbolic artificial intelligence}.

%\chapter*{Samenvatting}
%\addcontentsline{toc}{chapter}{Samenvatting}
%\setheader{Samenvatting}

%{\selectlanguage{dutch}

%Samenvatting in het Nederlands\ldots

%}


